Testing Criteria for Mobile Apps Based on Callback Sequences

App quality has been shown to be the most important indicator of app adoption. To assure quality, developers mainly use testing to find bugs in app and apply structural and GUI test coverage criteria. However, mobile apps have more behaviors than the GUI actions, e.g. an app also handles events from sensors and executes long-running background tasks through Android API calls to Services and AsyncTasks. Our studies found that there are important app behaviors via callback interactions that should be covered in testing, as data sharing between callbacks is common and is the cause of many existing bugs. We design a family of test criteria based on callback sequences and use the Callback Control Flow Automata (CCFA) to measure the coverage for testing. Our experiments show that guiding by our criteria, testing can find more bugs and trigger bugs faster than the state-of-the-art tools.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigconf-xelatex.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-sigconf-xelatex.pdf:  sample-sigconf-xelatex.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	xelatex $<
	- bibtex $*
	xelatex $<
	xelatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do xelatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigconf-xelatex.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> computing.tex <==
\section{Computing Coverage Criteria}\label{sec:computing}
To compute the coverage criteria C1, we can traverse the CCFA using a Breath First Search (BFS) traversal just by filtering callbacks depending on the context in which they are executed (an external event or an API call). Algorithm \ref{alg:computeseqeunces} shows the traversal to compute the different coverage criteria. It takes a CCFA for an app and the number of callbacks for each sequence and returns set of sequences for coverage criteria C1 and C2 callbacks. 

\begin{algorithm}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\SetAlgoLined
	\Input{$\mathit{CCFA}$}
	\Output{$\mathit{C1}$ set of sequences}
	
	
	% functions
	\SetKwFunction{UpdateSequences}{getSequences}
	\SetKwFunction{CallNode}{callNode}
	\SetKwFunction{TargetState}{targetState}
	\SetKwFunction{Propagate}{propagate}
	\SetKwFunction{Remove}{remove}
	\SetKwFunction{InitialState}{initialState}
	\SetKwFunction{GetContext}{getContext}
	
	% data elements
	\SetKwData{Workset}{Q}
	\SetKwData{Visited}{V}
	\SetKwData{Stack}{$CS_s$}
	\SetKwData{StackTarget}{$CS_t$}
	\SetKwData{Co}{C1}
	\SetKwData{Ct}{C2}
	\SetKwData{GUI}{GUI}	
	\SetKwData{Async}{EVENT}
	\SetKwData{Msg}{API\_ASYNC}
	\SetKwData{Call}{API\_SYNC}
	\SetKwData{GUIEvent}{GUI\_EVENT}
	\SetKwData{Point}{p}
%	\SetKwData{Call}{CALL}
	\SetKwData{Context}{$\mathit{cntx_s}$}	
	\SetKwData{ContextTarget}{$\mathit{cntx_t}$}	
	%	\SetKwData{ContextNew}{$\mathit{context_{new}}$}	
	\SetKwData{Cos}{$C1_{s}$}
	\SetKwData{CosTarget}{$C1_{t}$}

	\SetKwData{Cts}{$C2_{s}$}
	\SetKwData{GUIs}{$GUI_{s}$}
	\SetKwData{Con}{$C1_{n}$}
	\SetKwData{Ctn}{$C2_{n}$}
	\SetKwData{GUIn}{$GUI_{n}$}
	\SetKwData{si}{$s_i$}
	\SetKwProg{Fn}{procedure}{ \{} {\} }
	
	%  \Fn{COMPUTE\_SEQUENCES($CCFA$, $\mathit{n}$)}{	
	\si $ \leftarrow $ \InitialState{$CCFA$}\;
	add $($\si, $\{\}, $ \Async$, \{\})$ to \Workset\ and \Visited;
	
	%	\ForEach{$t \in $ transitions from initial state $CCFA$}{
	%		$n_0 \leftarrow $ \Entry{$ICFGs, t.i$}\;
	%		add $(n_0, x_0, t.s_2, null, t.i)$ to \Workset; $H[n_0, x_0] \leftarrow x_0$
	%	}
	\While{\Workset $\neq \emptyset$}{
		remove $(s,$, \Cos, \Context, \Stack$)$ from \Workset; 
		
		\ForEach{$t \in $ transitions from $s$ in $CCFA$}{
			
			(\ContextTarget, \StackTarget) $\leftarrow$ \GetContext{$t$, \Context, \Stack}\;
			\If{\ContextTarget $=$ \Async}{
				(\CosTarget, \Con) $\leftarrow$ \UpdateSequences{$t$, \Cos}\;
				\Co $\leftarrow$ \Co $\cup$ \Con
			}
%			\If{\Context $=$ \Call}{
%				(\Cts, \Ctn) $\leftarrow$ \UpdateSequences{$t$, $n$, \Cts}\;
%				\Ct $\leftarrow$ \Ct $\cup$ \Ctn
%			}
%			\If{\Context $=$ \Async or \GUIEvent}{
%				(\Cts, \Ctn) $\leftarrow$ \UpdateSequences{$t$, $n$, \Cts}\;
%				\Ct $\leftarrow$ \Ct $\cup$ \Ctn
%			}
			
			$\mathit{s_{t}} \leftarrow$  \TargetState{$t$}\;
			\If{$(\mathit{s_{t}}, $ \CosTarget, \ContextTarget, \StackTarget$) \notin $ \Visited}{
				add $(\mathit{s_{t}}, $ \CosTarget, \ContextTarget, \StackTarget$)$ to \Workset and \Visited;
			}
		}
	}
	
	\Return \Co
	% }
	
	\caption{Compute Sequences of Callbacks for coverage criterion C1 from the CCFA}
	\label{alg:computeseqeunces}
\end{algorithm}


Each element stored in the queue $\mathit{Q}$ and the set visited elements $\mathit{V}$ is a 4-tuple where the first element is a state in the CCFA; the second keep a set of incomplete sequences for C1; the third element is the current context in the CCFA; and the last element is a stack of contexts. The context is obtained from the guards in the transitions of the CCFA. If there is a transition with guard for an API call, the context is changed to API. The EVENT context is the default context and accounts for callbacks invoked in external events. Any other context is not considered in this algorithm

At line~2, the data structures $\mathit{Q}$ and $\mathit{V}$ are initialized with the initial state of the CCFA $\mathit{s_i}$, an empty set of sequences for C1, and the default EVENT context. For each transition out of the state $\mathit{s}$, we first compute the current context and update the context stack $\mathit{CS}$ (line~6). If the transition has a guard, then the new context is returned based on the guard and the current context is added to the stack. Otherwise, the current context and context stack are returned. In lines~7--10, new sequences for C1 are computed. The coverage criterion C1 includes all callbacks besides the one invoked in API calls. The function \inlinecode{getSequences} computes the new incomplete sequences ($\mathit{C1_t}$) and the sequences that reach the maximum length 2 ($\mathit{C1_{new}}$) using the input from the transition $\mathit{t}$. Lastly, at lines~11--14, we create the new tuple with the target state of the transition, $\mathit{s_t}$, and add it to the data structures $\mathit{Q}$ and $\mathit{V}$ if it is not present in $\mathit{V}$. This algorithm just computes sequences that involve callbacks invoked in external events. 


Algorithm \ref{alg:computec2} presents the traversal of the CCFA to generate callback sequences for C2. It is similar to Algorithm \ref{alg:computeseqeunces} to compute C1, but focusing on callbacks executed under the context of an API call. At line~8, we verify whether the previous context was not an API call which means that we should start new sequences from the previous callbacks points. The function \inlinecode{getPrevCallbacks} traverse the CCFA backwards from transitions $t$ and find the last callback input. Then, at line~10, new sequences are create with a previous callback point $c$ and the callback input in the transition $t$. For example, in Figure \ref{fig:ccfa} for the transition from $q_6$ to $q_7$ (contains a guard with an API call), the context changes from EVENT to API. The function \inlinecode{getPrevCallbacks} returns the callback input $A.onStart_{entry}$. Then, the function  \inlinecode{getSequences} would create the sequence of length 2 $A.onStart_{entry} \to L.onCreateLoader_{entry}$ as complete sequence for $C2_n$ and the sequence $L.onCreateLoader_{entry}$ as incomplete for $C2_t$. If the previous context was not different (lines 14--17), then we keep creating sequences between the callbacks invoked in the current API method. 

\begin{algorithm}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\SetAlgoLined
	\Input{$\mathit{CCFA}$}
	\Output{$\mathit{C1}$ set of sequences}
	
	
	% functions
	\SetKwFunction{UpdateSequences}{getSequences}
	\SetKwFunction{GetPrevCallbacks}{getPrevCallbacks}
	\SetKwFunction{CallNode}{callNode}
	\SetKwFunction{TargetState}{targetState}
	\SetKwFunction{Propagate}{propagate}
	\SetKwFunction{Remove}{remove}
	\SetKwFunction{InitialState}{initialState}
	\SetKwFunction{GetContext}{getContext}
	
	% data elements
	\SetKwData{Workset}{Q}
	\SetKwData{Visited}{V}
	\SetKwData{Stack}{$CS_s$}
	\SetKwData{StackTarget}{$CS_t$}
	\SetKwData{Co}{C1}
	\SetKwData{Ct}{C2}
	\SetKwData{GUI}{GUI}	
	\SetKwData{Async}{EVENT}
	\SetKwData{Msg}{API\_ASYNC}
	\SetKwData{Call}{API}
	\SetKwData{GUIEvent}{GUI\_EVENT}
	\SetKwData{Point}{p}
	%	\SetKwData{Call}{CALL}
	\SetKwData{Context}{$\mathit{cntx_s}$}	
	\SetKwData{ContextTarget}{$\mathit{cntx_t}$}	
	%	\SetKwData{ContextNew}{$\mathit{context_{new}}$}	
	\SetKwData{Cos}{$C1_{s}$}
	\SetKwData{CosTarget}{$C1_{t}$}
	
	\SetKwData{Cts}{$C2_{s}$}
	\SetKwData{CtsTarget}{$C2_{t}$}
	
	\SetKwData{GUIs}{$GUI_{s}$}
	\SetKwData{Con}{$C1_{n}$}
	\SetKwData{Ctn}{$C2_{n}$}
	\SetKwData{GUIn}{$GUI_{n}$}
	\SetKwData{si}{$s_i$}
	\SetKwProg{Fn}{procedure}{ \{} {\} }
	
	%  \Fn{COMPUTE\_SEQUENCES($CCFA$, $\mathit{n}$)}{	
	\si $ \leftarrow $ \InitialState{$CCFA$}\;
	add $($\si, $\{\},$ \Async$, \{\})$ to \Workset\ and \Visited;
	
	%	\ForEach{$t \in $ transitions from initial state $CCFA$}{
	%		$n_0 \leftarrow $ \Entry{$ICFGs, t.i$}\;
	%		add $(n_0, x_0, t.s_2, null, t.i)$ to \Workset; $H[n_0, x_0] \leftarrow x_0$
	%	}
	\While{\Workset $\neq \emptyset$}{
		remove $(s,$ \Cts, \Context, \Stack$)$ from \Workset; 
		
		\ForEach{$t \in $ transitions from $s$ in $CCFA$}{
			
			(\ContextTarget, \StackTarget) $\leftarrow$ \GetContext{$t$, \Context, \Stack}\;
			\If{\ContextTarget $=$ \Call}{
				\If{\ContextTarget $\neq$ \Context}{
					\ForEach{$c \in $ \GetPrevCallbacks{$t$}}{
						(\CtsTarget, \Ctn) $\leftarrow$ \UpdateSequences{$t$, $\{c\}$}\;
						\Ct $\leftarrow$ \Ct $\cup$ \Ctn	
					}
				}
				\Else{
					(\CtsTarget, \Ctn) $\leftarrow$ \UpdateSequences{$t$, \Cts}\;
					\Ct $\leftarrow$ \Ct $\cup$ \Ctn
				}
			
			%			\If{\Context $=$ \Call}{
			%				(\Cts, \Ctn) $\leftarrow$ \UpdateSequences{$t$, $n$, \Cts}\;
			%				\Ct $\leftarrow$ \Ct $\cup$ \Ctn
			%			}
			%			\If{\Context $=$ \Async or \GUIEvent}{
			%				(\Cts, \Ctn) $\leftarrow$ \UpdateSequences{$t$, $n$, \Cts}\;
			%				\Ct $\leftarrow$ \Ct $\cup$ \Ctn
			%			}
			
			$\mathit{s_{t}} \leftarrow$  \TargetState{$t$}\;
			\If{$(\mathit{s_{t}}, $ \CtsTarget, \ContextTarget, \StackTarget$) \notin $ \Visited}{
				add $(\mathit{s_{t}}, $ \CtsTarget, \ContextTarget, \StackTarget$)$ to \Workset and \Visited;
			}
		}
	}
}
	
	\Return \Ct
	% }
	
	\caption{Compute Sequences of Callbacks for coverage criterion C2 from the CCFA}
	\label{alg:computec2}
\end{algorithm}

In Algorithm \ref{alg:computec3}, we present how to generate sequences for coverage criterion C3. The algorithm first find all the transitions with a guard for an asynchronous callback in an API method call at line~1 (the CCFA uses the parameter $\mathit{msg}$). For each transition found $t \in M$, then \inlinecode{GetAsyncSeqs} returns all the possible sequences. \inlinecode{GetAsyncSeqs} first find the asynchronous callback that executes the API method in which the transition $t_{call}$ is found (line~8). This function traverses backward the CCFA until it reaches the entry point of the calling callback. Then, \inlinecode{findNextAsync} traverses the CCFA to find the reachable asynchronous transitions. For each reachable asynchronous transition, we generate sequences of length 3 (at line~12) with all the concurrent interleavings between the three callbacks.  

\begin{algorithm}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\SetAlgoLined

	\Input{$\mathit{CCFA}$}
	\Output{$\mathit{C3}$ set of sequences}
	
	\SetKwFunction{FindMsgTransitions}{findMsgTransitions}
	\SetKwFunction{FindCallerCallback}{findCallerCallback}
	\SetKwFunction{FindNextAsync}{findNextAsync}
	\SetKwFunction{GetAsyncSeqs}{GetAsyncSeqs}
	\SetKwFunction{GenerateSequences}{generateSequences}
	\SetKwData{Ct}{$C3$}
	\SetKwData{Ctc}{$C3_{call}$}
	\SetKwData{Caller}{c}
	\SetKwData{Async}{A}
	
	
    \SetKwProg{Fn}{procedure}{ \{} {\} }
	
	% find all msg transitions
	$M = $\FindMsgTransitions{CCFA}\;
	\ForEach{$t \in M$}{
		\Ct $\leftarrow$ \Ct $\cup$ \GetAsyncSeqs{$t$}
	}
	% find callbacks from msg transitions
	% for each callback call GetAsyncSeqs
	
	\Return \Ct
	
	\Fn{\GetAsyncSeqs($t_{call}$)}{
		\Ctc = \{\}\;
		\Caller $\leftarrow$ \FindCallerCallback{$t_{call}$}\;
		\Async $\leftarrow$ \FindNextAsync{$t_{call}$}\;
		\ForEach{$t \in $\Async}{
			\If{$t$ has guard for an external event}{
				\Ctc $\leftarrow$ \Ctc $\cup$ \GenerateSequences{$t_{call}$, \Caller, $t$}	
			}		
		}	 
	
		\Return \Ctc
    }
	
	% define GetAsyncSeqs
	\caption{Compute Sequences of for coverage criterion C3}\label{alg:computec3}
\end{algorithm}		



%To compute the coverage criterion C3, we need to include sequences with callbacks invoked asynchronously in API methods. However, the CCFA just keeps the order on which the asynchronous tasks to execute these callbacks are posted to event queue. We decided to compute the possible sequences of callbacks involving callbacks invoked asynchronously in API methods from the dynamic traces. In Algorithm \ref{alg:computec3}, the coverage criterion C3 takes all the sequences of callbacks in C2 (line~1) and add sequences from dynamic traces (lines~2--7). The algorithm generates sequences of $\mathit{n}$ callbacks where each callback invoked asynchronously in API methods is the last callback in the sequence (line~4) and the first (line~5). 
%
%\begin{algorithm}
%	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%	\SetAlgoLined
%	\Input{$\mathit{T}: $ complete traces, $\mathit{n}:$ number of callbacks per sequence, $C2: $ set of sequences}
%	\Output{$\mathit{C3}$ set of sequences}
%	
%	\SetKwFunction{FindPreviousCallbacks}{findPreviousCallbacks}
%	\SetKwFunction{FindNextCallbacks}{findNextCallbacks}
%	
%	\SetKwData{Co}{C3}
%	\SetKwData{Ct}{C2}
%	
%	\Co $ \leftarrow $ \Ct\;
%	\ForEach{$\mathit{t} \in \mathit{T}$}{
%		\If{$\mathit{t}$ is an API\_ASYNC callback and is an entry point}{
%			\Co $\leftarrow$ \Co $\cup$ \FindPreviousCallbacks{$\mathit{t}$, $\mathit{T}$, $\mathit{n}$}\;
%			\Co $\leftarrow$ \Co $\cup$ \FindNextCallbacks{$\mathit{t}$, $\mathit{T}$, $\mathit{n}$}
%		}
%	}
%	
%	\Return \Co
%	\caption{Compute Sequences of for coverage criterion C3}
%\label{alg:computec3}
%\end{algorithm}	


==> criteria-old.tex <==
\section{Designing Test Criteria Based on Callback Interactions}
In the above section, we have shown that it is important to consider callback interactions along different paths during testing. In this section, we first introduce a representation that displays all the possible callback sequences in an app, namely \textit{Callback Control Flow Automata} (CCFA) \cite{DaniloTSE19}. Using CCFA, we performed three studies to explore what are the important callback interactions we should test. We then designed a set of test criteria based on our findings.


%In this section we introduce new coverage criteria based on sequences of callbacks. We first introduce a representation to model the execution of Android apps using callbacks. Then, we performed three studies to understand how important to cover these interactions during testing. We finally present a set of test criteria based on our findings.

\subsection{Specifying Callback Sequences Using CCFA}
Event-driven, framework-based mobile apps base their implementation on callbacks provided by the Android framework's API methods. When an app is running, the framework executes the callbacks depending on the external events and the API calls made by the app. There exist 4 different changes of control between callbacks: 1) a callback $\mathit{B}$ is invoked synchronously after another callback $\mathit{A}$ is finished, 2) $\mathit{B}$ is invoked asynchronously after $\mathit{A}$, meaning that $\mathit{B}$ is put in the event queue after $\mathit{A}$, 3) during an execution of $\mathit{A}$, $\mathit{B}$ is invoked synchronously by an API call, and 4) during an execution of $\mathit{A}$, $\mathit{B}$ is invoked asynchronously by an API call, meaning that the API call puts $\mathit{B}$ in the event queue and the callback will be invoked eventually. 

To specify all possible sequences of callbacks generated from the 4 different changes of control between callbacks, we use \textit{Callback Control Flow Automata} (CCFA) \cite{DaniloTSE19}. A CCFA is a representation based on the \textit{Extended Finite State Machine} (EFMS) \cite{1600197}. In CCFAs, we use $\mathit{callbackname_{entry}}$ and $\mathit{callbackname_{exit}}$ as input symbols on the transitions. Each transition has a guard, specifying under which condition, the change of control between callbacks happen. These conditions can be about external events (an event handler callback cannot be executed unless an external event such as a GUI or sensing event occurs) or about API calls (the execution of a callback can also be made by an API method). % We use $\mathit{callbackname_{entry}}$ and $\mathit{callbackname_{exit}}$ as input symbols so we can specify the case where one callback is invoked during the execution of the other (see Type 3 and Type 4 of control flow discussed above).

\figref{ex} shows a simple Android app and its CCFA. The app has five callbacks.  The paths on the CCFA provides the possible sequences of these 5 callbacks. At the initial state $q1$, \inlinecode{onCreate()} from \inlinecode{class A} is invoked asynchronously when the event {\it launch} is triggered, noted by the transition $A.onCreate_{entry}, evt=launch$. This callback is followed synchronously by \inlinecode{onStart()} from \inlinecode{class A}. During the execution of \inlinecode{onStart()} , the API call \inlinecode{lm.initLoader(0, null, 1)} is invoked, which calls \inlinecode{onCreateLoader()} from \inlinecode{class L} synchronously (see transitions from $q4\rightarrow q_9$). At $q_5$, \inlinecode{onClick()} from \inlinecode{class CList} can be invoked asynchronously any number of times until  \inlinecode{onStop()} from \inlinecode{class A} is invoked. 


%\inlinecode{onStart()} from \inlinecode{class A} follows \inlinecode{onCreate()} from \inlinecode{class A} asynchronously.



%The CCFA shows a change of control from \inlinecode{A.onCreate()} to \inlinecode


%The CCFA shows a change of control from \inlinecode{A.onCreate()} to \inlinecode{A.onStart()} of type 1. Then, the transitions from $q_4$ to $q_6$ show a change of control from callback \inlinecode{A.onStart()} to \inlinecode{L.onCreateLoader()} of type 3. Note that the transition from the state $q_6$ to $q_7$ is guarded by a condition that checks whether the API call to \inlinecode{initLoader()} (at line 11 in \figref{examplecode}) was executed. Similarly, the transition from $q_5$ to $q_{10}$ is guarded by the execution of an event is represents a change of control of type 2. 


%{\color{red} change figure by adding different edges for async and sync}
\begin{figure}
	\centering
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\resizebox{0.85\columnwidth}{!}{
			%\lstset{basicstyle=\listingsfont, numbers=left, language=Java}
			\lstinputlisting{code/example2.java}
		}
		\caption{Source code of a simple Android app\label{fig:examplecode}}		
	\end{subfigure}
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\resizebox{\columnwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.3cm,
			semithick]
			%\tikzstyle{every state}=[fill=cadmiumgreen,draw=none,text=white]
			
			\node[initial,state, accepting] (Q1)                    {$q_1$};
			\node[state]         (Q2)  [above right=of Q1, xshift=-0.6cm] {$q_2$};
			\node[state]         (Q3)  [right of=Q2] {$q_3$};
			\node[state]         (Q4)  [right of=Q3] {$q_4$};
			\node[state]         (Q5)  [below of=Q3,xshift=0.7cm] {$q_5$};
			\node[state]         (Q6)  [right of=Q4] {$q_6$};
			%            \node[state]         (Q7)  [below of=Q4] {$q_7$};
			\node[state]         (Q8)  [below of=Q6] {$q_7$};
			\node[state]         (Q9)  [below of=Q8] {$q_{8}$};
			\node[state]         (Q10) [left of=Q9, xshift=-0.6cm] {$q_{9}$};
			\node[state]         (Q11) [below of=Q2, xshift=-0.7cm] {$q_{10}$};
			\node[state]         (Q12) [below of=Q5] {$q_{11}$};
			%    \node[state,accepting,double]         (J) [right of=I]       {$q_{10}$};
			
			\path
			(Q1) edge[edgeasync]         node[align=center] {($\mathit{A.onCeate_{entry}}$, \\  $\mathit{evt = launch}$)} (Q2)
			(Q2) edge          node[align=center] {($\mathit{A.onCreate_{exit}}$, \\ $\mathit{true}$)} (Q3)
			(Q3) edge          node[align=center] {($\mathit{A.onStart_{entry}}$, \\ $\mathit{true}$)} (Q4)
			(Q4) edge         node[align=right, near end] {($\mathit{A.onStart_{exit}}$, \\ $\mathit{true}$)} (Q5)
			edge          node[align=center] {$\epsilon$} (Q6)
			%(Q6) edge          node[align=center, left, near start] {($L.onCreateLoader_{entry}$, \\  TRUE)} (Q7)
			(Q6) edge          node[align=center,left, near start] {\footnotesize ($\mathit{L.onCreateLoader_{entry}}$, \\ \footnotesize $\mathit{cs=lm.initLoader()}$)} (Q8)
			
			%    (Q7) edge          node[align=right, left, near start] {($L.onCreateLoader_{exit}$, \\ TRUE)} (Q9)
			(Q8) edge          node[align=center,left, near end] {($\mathit{L.onCreateLoader_{exit}}$, \\ $\mathit{true}$)} (Q9)
			(Q9) edge          node[align=center] {$\epsilon$} (Q10)    
			(Q10) edge         node[align=left, right, very near end] {($\mathit{A.onStart_{exit}}$, $\mathit{true}$)} (Q5)
			
			(Q5) edge[edgeasync, bend left]         node[align=center,swap] {(\footnotesize $\mathit{CList.onClick_{entry}}$, \\ \footnotesize $\mathit{evt = click_{b1}}$)} (Q11)
			(Q11) edge[bend left]         node[align=center] {($\mathit{CList.onClick_{exit}}$, \\ $\mathit{true}$)} (Q5)
			(Q5) edge[edgeasync]     node[align=right, left] {($\mathit{A.onStop_{entry}}$, \\ $\mathit{evt = back\_button}$)} (Q12)
			(Q12) edge[bend left]     node[align=center] {($\mathit{A.onStop_{exit}}$, \\ $\mathit{true}$)} (Q1)
			%            (Q4) edge         node[align=center] {\scriptsize ($L.onCreateLoader_{entry}(cs)$, \\ \scriptsize $cs == initLoader$)} (Q5)
			%            (Q5) edge         node[align=center] {\scriptsize ($L.onCreateLoader_{exit}(cs)$, \\ TRUE)} (Q8)
			%            (Q8) edge         node[align=center,left] {($A.onStart_{exit}$, \\ TRUE)} (Q9)
			%            (Q9) edge[bend left]         node[align=center] {($A\$1.onClick_{entry}$(evt), \\ evt == click(b1))} (Q10)
			%            (Q10) edge[bend left]         node[align=center] {($A\$1.onClick_{exit}$(evt), \\ TRUE)} (Q9)
			%            (Q9) edge     node[align=center] {($A.onStop_{entry}$, \\ TRUE)} (Q11)
			%            (Q11) edge     node[align=center] {($A.onStop_{exit}$, \\ TRUE)} (Q1)
			;
			\end{tikzpicture}
		}
		\caption{A CCFA for simple app}\label{fig:ccfa}
	\end{subfigure}
	\caption{An example app and its CCFA}~\label{fig:ex}
\end{figure}

\subsection{What Important Callback Sequences We Should Test?}\label{sec:studies}
%To further understand what types of callback are important to test, we performed a set of studies.  For all the studies, we categorize the callbacks based on the context in which they are connected in the CCFA. The context is defined by the type of transition. For example, in Figure \ref{fig:ccfa}, the callbacks \inlinecode{A.onCreate()} and \inlinecode{A.onStart()} are executed under the context of the event \textit{launch}. Similarly, the callback \inlinecode{L.onCreateLoader()} is executed under the context of the API call \inlinecode{lm.initLoader()}. We define 3 types of callbacks based on the different kind of contexts found in the CCFA: \textit{EVENT} for callbacks invoked in external events such as GUI, GPS or power button, \textit{CALL} for callbacks invoked synchronously in API methods, and \textit{MSG} for callbacks invoked asynchronously in API methods (\eg the callback \inlinecode{onStartCommand} is executed asynchronously after calling \inlinecode{startService}). 

%We define the context based on the last guard seenThe source of execution for each callback can be an external event (\eg a GUI event, a GPS location update or a tab to the power button) or an API call. All callbacks invoked in external events are invoked asynchronously whereas an API method can execute a callback synchronously or asynchronously (\eg the callback \inlinecode{onStartCommand} is executed asynchronously after calling \inlinecode{startService}). Thus, we have three categories of callbacks: \textit{ASYNC} (asynchronous callbacks executed from external events), \textit{API\_SYNC} (synchronous callbacks executed in API methods) and \textit{API\_ASYNC} (asynchronous callbacks executed in API methods). In the studies, we want to verify whether a type of callback has important behavior that need to be tested. 

To answer this question, we designed two studies. In the first study, we investigate whether there exists dataflow between callbacks and what types of callbacks share dataflow. We believe that if there commonly exists dataflow between two callbacks, we need to test the inter-callback paths, as any incorrect definition or use of variables may only be exposed through exercising the inter-callback paths. In the second study, we explore whether there are bugs whose root causes are related to callback interactions and what types of callback interactions are likely buggy. We need to especially test such interactions of callbacks to avoid similar bugs in different apps. %Based on the three intuitions, we performed the following studies.

%Second, we want to investigate whether certain types of callbacks frequently invoked together. If so, we need to cover such callback sequences to ensure that the frequently occurred behaviors are well tested. Third,

% For example, a global object may be associated with a source and a sink that are located in different callbacks. To detect the bug where a source is missing or a sink is missing, we need to test the paths that traverse the callbacks.

\subsubsection{Study 1: Does there exist dataflow between callbacks? What types of callbacks share dataflow?} 

We performed a def-use analysis  for all the variables found on the CCFA on 55 apps randomly selected from the Google Play Market\footnote{\url{https://play.google.com}}. We report that an {\it inter-callback dataflow} is found when there is a definition whose use is in  a different callback.Our results show that all 55 apps contain inter-callback dataflow. Among all the def-use pairs we computed, 22.76\% are inter-callback. 

We performed further analysis to identify the type of callbacks in which def-use pairs are located. We found that 55\% of the inter-callback dataflow occurs between the callbacks that respond to external events, namely {\it event callbacks}. This is because the majority of the apps contain functionalities related to the GUI or the sensor components such as GPS or camera. The second most common (34\% of) inter-callback dataflow is located between synchronous callbacks invoked by the API method, namely {\it API\_SYNC callbacks}. This is because many API methods contain more than one synchronous callbacks, and it is common to share data in an API method. We also found def-use pairs between event callbacks and callbacks invoked in API methods, specially 7\% between event and API\_SYNC callbacks and 6\% between event and {\it API\_ASYNC} callbacks. API\_ASYNC are asynchronous callbacks invoked in the API method typically for responding to the {\it messages} from the API method. This interaction represents the scenario where the event handler invokes an API method and passes the data to the API method for handling the event. See Table~\ref{tab:dataflow} for the summary of our results.


% Lastly, 3\% of all dataflow was between synchronous and asynchronous callback invoked in API methods. 

%Finally, we also found that 4\% inter-callback dataflow is from an {\it event callback} to an asynchronous callback invoked in API methods. It is also a representative scenario where an event handler calls an API method, while many API methods implement message passing routines, and the asynchronous callbacks are invoked to handle the messages in the API method. %The rest of the possible combinations account just for 1\% or less.
\begin{table}[!ht]
	\centering
	\caption{Dataflow between callbacks. EV: event callback, AS: API\_SYNC callback, AA: API\_ASYNC callback}\label{tab:dataflow}
	%	\resizebox{\columnwidth}{!}{
	\begin{tabular}{|c|c|c|c|} \hline
		EV-EV & AS-AS & EV-AS & EV-AA  \\ \hline \hline
		55\% & 34\% & 7\% & 6\% \\ \hline
	\end{tabular}
	%	}
\end{table}


In addition, our study reports that although the global dataflow can propagate through maximum 18 callbacks, 38\% global dataflow are related to consecutive callbacks sequenced on CCFA.

%We also studied the number of callbacks it takes a def to reach a use in the CCFA. We found that most of the def-use pairs is between two contiguous callbacks (38\%). The maximum sequence of callback we found for a definition to be used was 18 and the median for all the apps was 2. Therefore, from the point of view of dataflow, most of the share of data is done between two contiguous callbacks.  
%which account for 34\% of all value flows. We observed that some API methods invoke more than one callback and the share of data between those callbacks is very common in apps. Value flows from callbacks EVENT $\to$ CALL and from callbacks ASYNC $\to$ MSG account for 4\% each one. The rest of the possible combinations account just for 1\% or less.

%\subsubsection{Study 2:  what types of callback sequences frequently occur in traces?} 
%We instrumented 5 apps, including \textit{ContactsList}, \textit{StandupTimer}, \textit{BARIA}, \textit{JustCraigslist} and \textit{OpenSudoku}. We collected a total of XXX MB of traces by testing the apps manually. We label the callbacks occurred the traces with the types of {\it event}, {\it API\_SYNC} and {\it API\_ASYNC}.  We then perform common sequence mining on the sequence of labels occurred on the traces. Our goal is to find the most frequent length 2 callback sub-sequence. Among such subsequence we found, 64\% are a pair of event callbacks and 21\% are a pair of  {\it API\_ASYNC} callbacks. This finding is consistent with our first study.


%then mine the most common sequences with two callbacks considering the type of callback. 

%{\bf RQ1:} We found that from that 64\% of the callbacks sequences include just EVENT callbacks. The rest of the interactions found in the traces account for 21\% between CALL callbacks. Similarly to the first study, most of the sequences mined are related to callbacks invoked in external events. 

\subsubsection{Study 2: What types of callbacks are likely buggy?} 

As a pilot study, we analyzed 1526 bugs from 6 apps. We identified the bugs that lead to crash and found that 26 of such bugs are related to callback interactions. That is, we need to exercise a sequence of callbacks cause the app to crash. Furthermore, we found that all the 26 bugs are related to 2 callbacks.  85\% of the bugs are related to the two consecutive callbacks specified in the CCFA. This data aligns with our findings from the first study that many of the time, there is data sharing at the neighbor callbacks in the execution paths. 

Our results are presented in Table \ref{tab:bugstudy}. The first column lists the apps we studied. Under {\it Bugs}, we show the number of bugs we inspected. Under {\it Multi-C}, we give the number of bugs whose root causes are related to multiple callbacks. Under  {\it EV-EV},  {\it AS-AS},  {\it EV-AS}  and {\it EV-AA}, we show what types of callback interactions that lead to the bug.  Our results show that there are 6 bugs related to interactions of two event handlers, 11 bugs are related to synchronous calls in the API method, and 13 bugs are caused by improper interactions between the event handler callbacks and the asynchronous callbacks in the API method. These bugs are mostly race conditions as a result of asynchronous invocations.





%The classification is based on the type of callbacks involve in the bug. The column \textit{Analyzed} shows the number of bugs we manually studied after filtering by keywords. The column \textit{Matched} shows the number of bugs that match our criteria for inter-callback bugs. Each of the following columns shows the type of callbacks involve in the bug with a total of 4 different combinations.

% We found that 6 of the inter-callback bugs involve just callbacks invoked in external events. The execution between callbacks invoked in external events and callbacks invoked in API methods is also important. We found a total of 19 bugs that involve these kind of callbacks, 6 between EVENT and API\_SYNC, and 13 between EVENT and API\_ASYNC. We also found bugs in which just asynchronous callbacks invoked in API method (API\_ASYNC) were involve, mostly race conditions between these callbacks. 

%We also found that for 85\% of the bugs, the callbacks involve in the bug were executed contiguously. This result also aligns with the results of the first study in which most of the dataflow was between two contiguous callbacks. 
%The column \textit{EVENT} contain the number of bugs which involve at least one callback of type EVENT. We apply the same metric for columns \textit{CALL} and \textit{MSG}. Most of the bugs reported under EVENT include both EVENT and MSG callbacks (they are also reported under MSG). We found just 2 bugs in which the callbacks involved were just of type EVENT. For bugs involving callbacks of type CALL, we found 2 bugs which also involve EVENT callbacks and 2 bugs which just involve CALL callbacks. 

\begin{table}[!ht]
	\centering
	\caption{Bug study results. EV: event callback, AS: API\_SYNC callback, AA: API\_ASYNC callback}\label{tab:bugstudy}
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{|l||c|c||c|c|c|c|} \hline
			App & Bugs & Multi-C & EV-EV & AS-AS & EV-AS & EV-AA  \\ \hline \hline
			ConnectBot & 9 & 5 & 1 & 2 & 0 & 2  \\ \hline
			FileDownloader & 12 & 2 & 0 & 1 & 1 & 0  \\ \hline
			AntennaPod & 133 & 5 & 1 & 1 & 0 & 4  \\ \hline
			cgeo & 273 & 4 & 2 & 1 & 0 & 3  \\ \hline
			Wordpress & 315 & 5 & 1 & 0  & 2 & 2  \\ \hline
			Ankidroid & 784 & 5 & 1 & 2 & 1 & 2  \\ \hline
			\textbf{Total} & \textbf{1526} & \textbf{26} & \textbf{6} &  \textbf{7} & \textbf{4} & \textbf{13}  \\ \hline
		\end{tabular}
	}
\end{table}
%Note that if the bug requires callback interactions \textit{(Asynchronous, Follows)} and \textit{(Synchronous,Follows)} we categorize it as the behavior to trigger the bug can be cover by C1. If the bug includes an \textit{(Synchronous, Invocation)} interaction, then we categorize it as C2. Lastly, if the bug includes an \textit{(Asynchronous, Invocation)}, the behavior can only be covered by C3. 

%\begin{table}[!ht]
%	\centering
%	\caption{Bug Study Results}\label{tab:bugstudy}
%		\resizebox{\columnwidth}{!}{
%	\begin{tabular}{|l|r|r|r|r|r|} \hline
%		App & Analyzed & Matched & EVENT & CALL & MSG \\ \hline \hline
%		ConnectBot & 9 & 5 & 2 & 0 & 4 \\ \hline
%		FileDownloader & 12 & 2 & 1 & 1 & 1 \\ \hline
%		AntennaPod & 133 & 5 & 4 & 0 & 5 \\ \hline
%		cgeo & 273 & 4 & 2 & 0 & 4 \\ \hline
%		Wordpress & 315 & 5 & 1 & 2 & 2 \\ \hline
%		Ankidroid & 784 & 5 & 2 & 1 & 4 \\ \hline
%		\textbf{Total} & \textbf{1526} & \textbf{26} & \textbf{12} &  \textbf{4} & \textbf{20} \\ \hline
%	\end{tabular}
%		}
%\end{table}

%{\bf RQ1:} Inter-callback bugs were frequent among all apps. We found a total of 26 bugs related to inter-callbacks apps in 1526 bugs studied. 

%{\bf RQ2:} Our results shows that most of the bugs found include callbacks invoked asynchronously in API methods. Most of these bugs are race conditions between other callbacks of type API\_ASYNC or callbacks of type EVENT. We also found that for some cases, callbacks invoke synchronously can also be prompt to faults.  

%The most relevant interactions were EVENT callbacks. We see that the main cause of these bugs is the lack of knowledge of all possible callback paths that can be executed when there are other asynchronous callbacks. 

\subsubsection{Conclusions of the Studies.} 

From the study, we learned that although it is beneficial to test long callback sequences, the priority is to thoroughly cover neighbor callback interactions, starting with a length of two callbacks.

First, we want to test interactions between event callbacks as these callbacks share data and they occupy the main behavior of apps. Second, synchronous callbacks invoked in the API methods are typically not targeted by any GUI testing tools; however, there are data sharing and many bugs related to such callbacks. We want to trigger these callbacks in testing. Finally, a main source of callback interaction bugs go to race conditions caused by asynchronous invocations. We need to well test the interleaves of relevant callbacks. In the following, we show the testing criteria we designed based on these findings.


%In the study 1 we found that the most of the data is shared between callbacks involve callbacks invoked in external events or windows (EVENT type). This tells us that the majority of the app implementation is related to GUI (including windows and GUI event handlers) and external events related to components of the phone such as GPS, camera, etc. However, our bug study shows that the callbacks invoke in API methods are prompt to introduce faults. Callbacks invoke asynchronously in API methods are prompt to introduce concurrency faults. Sequences of methods (specially pair of methods) have been used before for coverage criteria designed to detect concurrency bugs \cite{choudharyconcurrency, tasharoficoncurrency}. Thus, we consider that callback sequences are an adequate metric to cover concurrency faults in Android apps. 

%We design different coverage criteria based on the results founded in our studies. Since most of the data shared between callbacks and the most common interactions among apps include just callbacks of type EVENT, we design a coverage criterion that include callbacks of type EVENT. Because some of the faults found include both EVENT and API\_SYNC or EVENT and API\_ASYNC types of callbacks, we design coverage criterion to model these interactions also. We also decide to compute sequences of length 2 because most of the results found in the studies involve contiguous callbacks. 

%\subsection{Designing Testing Criteria Based on Callback Interactions}
%We have identified 3 types of callbacks based on the control change between two callbacks. We have used examples to show these interactions are feasible. In this section, we develop three testing criteria, namely {\it C1}, {\it C2} and {\it C3}, that aim to cover these interactions. Shown in Table \ref{tab:coveragecriteria}, the criteria is designed in a way that {\it C1} is the weakest, {\it C2} is stronger by including one more type of callbacks, and {\it C3} is the strongest that aim for covering all types of callbacks.
% In the following, we further show that there are different sets of app behaviors that can be covered by C1, C2 and C3. 

%The main hypothesis of this paper is that current GUI event-based and structural coverage criteria are not the best metrics to verify the adequacy of a test suite. We want to test the hypothesis that a more specialized coverage criteria is needed besides GUI event-based ones. We design 3 coverage criteria, one more complex than the other to observe whether the behaviors added are important to identify faults. Each coverage criterion is defined based on the type of callbacks interactions they cover. Table \ref{tab:coveragecriteria} shows the 3 different coverage criteria we define and the callbacks interaction that each of them cover. 

%Each coverage criterion is defined based on type of interactions they cover. 

%Therefore, by covering just certain changes of control between callbacks, a coverage criterion focus on specific behaviors in the app. Table \ref{tab:coveragecriteria} shows 4 coverage criteria we define. 



\subsection{Testing Criteria Based on Callback Interactions}
%We have identified 3 types of callbacks based on the control change between two callbacks. We have used examples to show these interactions are feasible and studies to find the most important interactions. In this section, we develop three testing criteria, namely {\it C1}, {\it C2} and {\it C3}, that aim to cover these interactions. All of the coverage criteria define here are based on callback sequences. We formally define callback sequences before introducing C1, C2 and C3. The length of a callback sequence is identified by the number of callbacks involve in a sequence. 

Here, we present three testing criteria, namely $C1$, $C2$ and $C3$. In the following, we first formally introduce the concept of {\it callback sequence}. It is used to define the three criteria. 
%{\color{red} to modify: C1, C2 and C3 are getting stronger and stronger, $C1\subseteq C2$ and $C2\subseteq C3$}

\begin{mydef}[Callback Sequence]
	Let $C = \{c1, c2, ..., cn\}$ the callbacks implemented for an app $P$. The input symbols of the CCFA for $P$ are defined by the set $I = \{c1_{entry}, c1_{exit}, c2_{entry}, c2_{exit}, ..., cn_{entry}, cn_{exit}\}$. A {\it callback sequence} is $\langle s1 \to s2 \to ...\to sm \rangle$ where $si \in I$ for $1 \leq i \leq m$. The {\it length} of a callback sequence is the number of callbacks $c$, or in another word, the number of the input symbol $c_{entry}$ the sequence contains.
\end{mydef}

%We introduce each of the coverage criterion and present examples for their understanding:
% A callback sequence of length 2 (two callbacks), include 1 callback interaction in the sequence. 
%\begin{mydef}[Callback Interaction]
%	A callback interaction represent the change of control from one callback to another. There are two types of callback interaction, \textit{invocation} and \textit{follows}. Let $A$ and $B$ be two callbacks implemented in an app $P$. An invocation callback interaction between $A$ and $B$ is defined by the sequence $\langle A_{entry} \to B_{entry} \rangle$ where the callback $B$ is invoked synchronously by an API call made in $A$. A follows callbacks interaction $A$ and $B$ is defined by the sequence $\langle A_{exit} \to B_{entry} \rangle$ and represents the execution of $B$ after the execution of $A$ finishes. 
%\end{mydef}



%Shown in Table \ref{tab:coveragecriteria}, the criteria is designed in a way that {\it C1} is the weakest, {\it C2} is stronger by including one more type of callbacks, and {\it C3} is the strongest that aim for covering all types of callbacks.
% In the following, we further show that there are different sets of app behaviors that can be covered by C1, C2 and C3.

%The main hypothesis of this paper is that current GUI event-based and structural coverage criteria are not the best metrics to verify the adequacy of a test suite. We want to test the hypothesis that a more specialized coverage criteria is needed besides GUI event-based ones. We design 3 coverage criteria, one more complex than the other to observe whether the behaviors added are important to identify faults. Each coverage criterion is defined based on the type of callbacks interactions they cover. Table \ref{tab:coveragecriteria} shows the 3 different coverage criteria we define and the callbacks interaction that each of them cover.

%Each coverage criterion is defined based on type of interactions they cover.

%Therefore, by covering just certain changes of control between callbacks, a coverage criterion focus on specific behaviors in the app. Table \ref{tab:coveragecriteria} shows 4 coverage criteria we define.

%\begin{table}
%	\centering
%	\caption{Testing Criteria based on Callback Interactions}\label{tab:coveragecriteria}
%	%    \resizebox{\columnwidth}{!}{
%	\begin{tabular}{|l|l|} \hline
%		Name & Callback Types  \\ \hline  \hline
%		C1 & EVENT \\ \hline
%		C2 & EVENT, CALL \\ \hline
%		C3 & EVENT, CALL, MSG  \\ \hline
%	\end{tabular}
%	%    }
%\end{table}

\subsubsection{C1}
Coverage criterion C1 is designed to cover callback interactions related to event callbacks. The events can be a GUI event or the events from the sensing components. 

\begin{mydef}[C1]\label{def:c1}
	Let $C = \{c1, c2, ..., cn\}$ the callbacks implemented for an app $P$.  Let $E \subseteq C$ be the set of callbacks for handling events in an app $P$. Let $E_{I}$ be the set of input symbols (the entry and exit points) for any callback $c \in E$. A coverage criterion C1 is satisfied if and only if for all callback sequences of length 2,  $\langle s1 \to s2 \to s3\rangle$, where $s1,s2,s3 \in E_{I}$, generated from the CCFA of $P$, the traces $T$ contain $S$. 
\end{mydef}

The behaviors required to be covered by C1 are close to the behaviors covered by GUI testing tools~\cite{guiripper}. The difference is that C1 also requires to exercise the interactions between callbacks invoked in other kind of external events besides GUI events. As an example, in Figure \ref{fig:example3}, the app registers the listener callbacks for two buttons at lines~7 and 8, and a callback to receive GPS location updates at line~9. Figure \ref{fig:ccfaexample3} shows the CCFA built for the app. Given C1, we generate the following sequences of callbacks for \inlinecode{A.onCreate()}:
\begin{enumerate}
	\item $\mathit{A.onCreate_{entry}} \to \mathit{A.onCreate_{exit}} \to$ \\ $\mathit{Button1.onClick_{entry}}$
	\item $\mathit{A.onCreate_{entry}} \to \mathit{A.onCreate_{exit}} \to$ \\ $\mathit{Button2.onClick_{entry}}$
	\item $\mathit{A.onCreate_{entry}} \to \mathit{A.onCreate_{exit}} \to$ \\ $\mathit{LocList.onLocationUpdate_{entry}}$
\end{enumerate}

Using a similar approach, we can generate the callback sequence centered on \inlinecode{Button1.onClick} (including 2 sequences), \inlinecode{Button2.onClick} (2 sequences) and \inlinecode{LocList.onLocationUpdate} (2 sequences). As a result, we have a total of 9 (3+2+2+2) callback sequences to cover. To satisfy C1 for this app, we need to ensure that testing covers the cases where the  location events happen before or after a GUI callback. Whereas, any GUI based coverage criterion just need to cover the combination of the GUI callbacks. %Therefore, C1 ca more behaviors to test.

\begin{figure}
	\centering
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\resizebox{0.85\columnwidth}{!}{
			%\lstset{basicstyle=\listingsfont, numbers=left, language=Java}
			\lstinputlisting{code/example3.java}
		}
		\caption{Source code of a simple Android app including the GPS event\label{fig:example3}}       
	\end{subfigure}
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\resizebox{0.85\columnwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.3cm,
			semithick]
			%\tikzstyle{every state}=[fill=cadmiumgreen,draw=none,text=white]
			
			\node[initial,state, accepting] (Q1)                    {$q_1$};
			\node[state]         (Q2)  [below of=Q1] {$q_2$};
			\node[state]         (Q3)  [below of=Q2] {$q_3$};
			\node[state]         (Q4)  [left of=Q3, xshift=-0.9cm] {$q_4$};
			\node[state]         (Q5)  [right of=Q3, xshift=0.9cm] {$q_5$};
			\node[state]         (Q6)  [below of=Q3,yshift=-0.9cm] {$q_6$};
			
			\path
			(Q1) edge         node[align=center] {(\footnotesize $\mathit{A.onCeate_{entry}}$, $\mathit{evt = launch}$)} (Q2)
			(Q2) edge          node[near start] {(\footnotesize $\mathit{A.onCreate_{exit}}$, $\mathit{true}$)} (Q3)
			%           
			(Q3) edge[edgeasync, bend right,swap]          node[align=center] {(\footnotesize $\mathit{Button1.onClick_{entry}}$, \\ \footnotesize $\mathit{evt = click_{b1}}$)} (Q4)
			(Q4) edge[bend right, swap]          node[align=center] {(\footnotesize $\mathit{Button1.onClick_{exit}}$, \\ \footnotesize true)} (Q3)
			
			(Q3) edge[edgeasync, bend left]          node[align=center] {(\footnotesize $\mathit{Button2.onClick_{entry}}$, \\ \footnotesize $\mathit{evt = click_{b2}}$)} (Q5)
			(Q5) edge[bend left]          node[align=center] {(\footnotesize $\mathit{Button2.onClick_{exit}}$, \\ \footnotesize $\mathit{true}$)} (Q3)
			
			(Q3) edge[edgeasync, bend right, swap]          node[align=center,near end] {(\footnotesize $\mathit{LocList.onLocationUpdate_{entry}}$, \\ \footnotesize $\mathit{evt = location}$)} (Q6)
			(Q6) edge[bend right, swap]          node[align=center,near start] {(\footnotesize $\mathit{LocList.onLocationUpdate_{exit}}$, \\ \footnotesize $\mathit{true}$)} (Q3)
			;
			\end{tikzpicture}
		}
		\caption{A CCFA for the app}\label{fig:ccfaexample3}
	\end{subfigure}
	\caption{An app with Location Callbacks}\label{fig:applocation}
\end{figure}


\subsubsection{C2}
Coverage criterion C2 focuses to trigger the callback interactions related to synchronous callbacks implemented in the API methods (API\_SYNC). Specifically, there are two types of sequences that we aim to test: 1)  a synchronous callback in the API method and the caller of the API method which is an event callback, and 2) two synchronous callbacks in the same API method. For example, in Figure~\ref{fig:ccfa}, we aim to test the sequence $\mathit{A.onStart_{entry}} \to \mathit{L.onCreateLoader_{entry}}$.  In Figure \ref{fig:filedownloader610subseq}, we will test  $\mathit{DBHelper.onCreate_{exit}} \to \mathit{DBHelper.onOpen_{entry}}$ and  $\mathit{DBHelper.onUpgrade_{exit}} \to \mathit{DBHelper.onOpen_{entry}}$. All these callbacks are synchounous callbacks implemented in the API method \inlinecode{dbh.getWritableDatabase()} at line~5 in Figure~\ref{fig:filedownloder610code}.

\begin{mydef}[C2]
	Let $Z =\{c1, c2, ..., cn\}$ and $Z \subseteq C$ be the set of callbacks of type API\_SYNC in an app $P$, and $Z_{I}$ be the set of input symbols  (the entry and exit points) for any callback $c \in Z$. Let $E \subseteq C$ be the set of callbacks for handling events in an app $P$, and $E_{I}$ be the set of input symbols (the entry and exit points) for any callback $c \in E$. A coverage criterion C2 is satisfied if and only if for all call sequences of length 2,  $\langle s1 \to s2 \rangle$, where $s1 \in E_I$ or $s1\in Z_{I}$ and $s2 \in Z_{I}$, generated from the CCFA of $P$, the traces $T$ contain $S$. 	
\end{mydef}



%To generate sequences involving API\_SYNC callbacks, we can use the CCFA. For example, from the callback \inlinecode{A.onStart} shown in the CCFA in Figure \ref{fig:ccfa}, there are 3 sequences of callbacks of length 2 that can be generated:
%\begin{itemize}
%	\item $\mathit{A.onStart_{entry}} \to \mathit{L.onCreateLoader_{entry}}$
%	\item $\mathit{A.onStart_{entry}} \to \mathit{A.Start_{exit}} \to \mathit{A.onStop_{entry}}$
%	\item $\mathit{A.onStart_{entry}} \to \mathit{A.Start_{exit}} \to \mathit{CList.onClick_{entry}}$
%\end{itemize}

This test criterion requires to trigger the API method as well as the synchronous call(s) in the API method. Sometimes, there exist different callback sequences in the API method dependent on the state of the system when the API call is made. C2 requires to test all possible callback sequences. In Figures \ref{fig:filedownloder610code} and \ref{fig:filedownloader610subseq}, we will test all the following callback sequences from  \inlinecode{FDService.onCreate()}:
\begin{enumerate}
	\item $\mathit{FDService.onCreate_{entry}} \to \mathit{DBHelper.onCreate_{entry}}$
	\item $\mathit{FDService.onCreate_{entry}} \to$ \\ $\mathit{DBHelper.onUpgrade_{entry}}$
	\item $\mathit{FDService.onCreate_{entry}} \to \mathit{DBHelper.onOpen_{entry}}$
\end{enumerate}

The states that can trigger these callback sequences include (1) the app is just installed, (2) the app is just updated from an older version previously installed on the phone, and (3) the app is running without any installation and upgrading. That is, in this example, we even need to prepare special environments to satisfy C2.


%To satisfy this criterion, need to reach at least all API methods that invoke callbacks. For example, in Figures \ref{fig:examplecode} and \ref{fig:ccfa} since in the callback \inlinecode{A.onStart()} there is a path in the app in which \inlinecode{A.onStart()} does not call \inlinecode{LoaderManager.initLoader()}. Therefore, a test suite covering executions of callback  \inlinecode{A.onStart()} does not imply covering all sequences in C2 related to \inlinecode{A.onStart()}. 

%Even when a test suite reaches an API call that invokes callbacks synchronously, there are some cases in which the API method can execute different callbacks under different states of the system. As we presented in the example showed 

%To completely test these sequences, the app has to be freshly installed and also has to update an older version of the app previously installed in the phone. Thus, to satisfy C2, apps have to be tested under special environments.

\subsubsection{C3} The API methods can make asynchronous calls include \inlinecode{Handler.sendMessage} and \inlinecode{Context.startService}, which will trigger asynchronous callbacks  (we call them API\_ASYNC). The past studies ~\cite{raceandroidmaiya, raceandroidhsiao, racebielik} as well as our own bug study presented in Section \ref{sec:studies} all show that asynchronous callbacks invoked in API calls can lead to concurrency bugs. Such bugs typically involve two event calls and one asynchronous call. 

\begin{figure}
	\centering
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\includegraphics[width=0.9\columnwidth]{figures/eventqueue1.eps}
		\caption{Event Queue for first scenario}\label{fig:eventqueue1}
	\end{subfigure}
	
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\includegraphics[width=0.9\columnwidth]{figures/eventqueue2.eps}
		\caption{Event Queue for second scenario}\label{fig:eventqueue2}
	\end{subfigure}
	\caption{The behavior of the event queue for two different scenarios in the appp chanu}\label{fig:eventqueues}
\end{figure}

We focus on the scenarios that can happen when an asynchronous callback invokes an API method that schedules the execution of another asynchronous callback (API\_ASYNC). We use the example presented in in Figures \ref{fig:chanu140code} and \ref{fig:chanu140subseq} to represent the behaviors that need to be covered to satisfy C3. As we mentioned in Section \ref{sec:motivation}, the two main scenarios in this app depend on whether the user double tabs the button to take the picture or not. 

In Figure \ref{fig:eventqueues} we present the event queue behavior for both scenarios. Each scenario shows the tasks that the event queue has a three different times during the execution of the app. In the first scenario (Figure \ref{fig:eventqueue1}), the user tabs the click button and the system schedules to execute \inlinecode{CaptureList.onClick()} (step 1). When \inlinecode{CaptureList.onClick()} invokes \inlinecode{takePicture()}, it schedules a task to execute \inlinecode{CamAct\$3.onPictureTaken()} (step 2). Then, the user tabs again the click button to take another picture (step 3). In the second scenario (Figure \ref{fig:eventqueue2}), the user double tabs the click button, thus, the system schedules two tasks to execute the callback \inlinecode{CaptureList.onClick()} (step 1). Then, the API method \inlinecode{takePicture()} schedules a task to execute the callback \inlinecode{CamAct\$3.onPictureTaken()} (step 2), but is is executed after \inlinecode{CaptureList.onClick()} (in step 3). This two scenarios generate the following sequences:  
\begin{enumerate}
	\item $\mathit{CaptureList.onClick_{exit}} \to$ \\ $\mathit{CamAct\$3.onPictureTaken_{entry}}$ \\ $\mathit{CamAct\$3.onPictureTaken_{exit}}$ \\ $\mathit{CaptureList.onClick_{entry}}$
	\item $\mathit{CaptureList.onClick_{exit}} \to$ \\ $\mathit{CaptureList.onClick_{entry}}$ \\ $\mathit{CaptureList.onClick_{exit}}$ \\ $\mathit{CamAct\$3.onPictureTaken_{entry}}$
\end{enumerate}


We developed a function, namely $\mathit{GetAsyncSeqs(c)}$, that takes an API\_ASYNC as an input and traverses the CCFA to identify all possible interleavings between $c$ and its event callbacks that potentially concurrently run with $c$.  For example, in Figures \ref{fig:chanu140code} and \ref{fig:chanu140subseq} callbacks that cover all the different interleavings from the scenarios for each callback executed asynchronously in API methods $c$. We focus on the scenarios that involves two asynchronous callbacks invoked in external in which one of them invokes an API method that schedules the execution of a callback. The algorithm starts by identifying API\_ASYNC callbacks from API methods invoked in EVENT callbacks. It then, identifies the next possible asynchronous callbacks of type EVENT in the CCFA and generate the sequences from the two scenarios presented. 

%named $\mathit{GetAsyncSeqs(c)}$, that for each callback executed asynchronously in API methods $c$, it returns the set of sequences involving the different interleavings of callbacks related to the execution $c$. 

%For example, in Figures \ref{fig:chanu140code} and \ref{fig:chanu140subseq}, there can be the following two interleavings for the callbacks \inlinecode{CaptureList.onClick()} and \inlinecode{CamAct\$3.onPictureTaken}:
%
%\begin{enumerate}
%	\item $\mathit{CaptureList.onClick_{exit}} \to$ \\ $\mathit{CamAct\$3.onPictureTaken_{entry}}$ \\ $\mathit{CamAct\$3.onPictureTaken_{exit}}$ \\ $\mathit{CaptureList.onClick_{entry}}$
%	\item $\mathit{CaptureList.onClick_{exit}} \to$ \\ $\mathit{CaptureList.onClick_{entry}}$ \\ $\mathit{CaptureList.onClick_{exit}}$ \\ $\mathit{CamAct\$3.onPictureTaken_{entry}}$
%\end{enumerate}
%
%In the first case, there is not other tasks in the event queue when the task of executing \inlinecode{CamAct\$3.onPictureTaken()} was posted by \inlinecode{takePicture()}. As a result, \inlinecode{CamAct\$3.onPictureTaken()} is executed after \inlinecode{CaptureList.onClick()}, and any asynchronous callback will be executed after \inlinecode{CamAct\$3.onPictureTaken()} (in this case \inlinecode{CaptureList.onClick()}). In the second case, the second \inlinecode{CaptureList.onClick()} follows right after the first one before \inlinecode{takePicture()} posts the task of \inlinecode{CamAct\$3.onPictureTaken()}. The implementation of the app does not prepare for such case and can lead to crash. During testing, we should consider all possible such interleavings to help expose such problems.
%
%%These kind of interleavings are important to test in order to detect concurrency bugs in Android apps. 

%named $\mathit{GetAsyncSeqs(c)}$, that for each callback executed asynchronously in API methods $c$, it returns the set of sequences involving the different interleavings of callbacks related to the execution $c$. 

%In the CCFA, callbacks invoked asynchronously in API methods appear where the callbacks is enqueued to the event queue and not where the callbacks are actually executed at runtime. Therefore, we cannot compute the callback sequences for C3 just by traversing the CCFA. To compute these sequences, we use the function $\mathit{GetAsyncSeqs(c)}$ which receives an API\_ASYNC callback $c$ and returns all the possible sequences of length 2 involving callback $c$ and any other feasible API\_ASYNC and EVENT callback.  

\begin{mydef}[C3]
	Let $Y =\{c1, c2, ..., cn\}$ and $Y \subseteq C$ be the set of callbacks of type API\_ASYNC. Let $Y_{I}$ include the entry and exit points of each callback $c \in Z$.
	A coverage criterion C3 is satisfied by callback traces $T$ if and only if for all sequences of length 3, $S = \langle s1, s2, s3, s4 \rangle$ (where $s1, s2, s3, s4 \in Z \cup E$) generated from the function $\mathit{GetAsyncSeqs(c)}$ for each $c \in Y$, $T$ contains $S$. 
\end{mydef}
%For example, in the issue \#3991 for the app \textit{cgeo}~\cite{cgeo3991}, there is data race condition between a tab to the back button and an asynchronous callback executed using the API method \inlinecode{Handler.sendMessage}. Thus, the asynchronous interactions between external events and also between callbacks invoke in API calls are important to cover.

C3, similarly to C1, cover different interleavings of asynchronous callbacks. To satisfy C1, a test suite has to cover different interleaving of asynchronous callbacks invoked in external events. C3 aims to test concurrent behavior that involves the execution of an asynchronous callback invoked in API methods. As the example we presented shows, API\_ASYNC callbacks can interact different feasible callbacks executed in external events.  

%C3 aims to test concurrent behavior that an app can present from not just external events, but the interaction of external events and callbacks invoked asynchronously in API methods. 

%We present an algorithm for $\mathit{GetAsyncSeqs(c)}$ Section \ref{sec:computing}. 


==> criteria.tex <==
\section{Defining Testing Criteria Based on Callback Interactions}
We analyzed potential interactions that can exist between two callbacks in Android apps. We performed three studies to understand how important to cover these interactions during testing. We finally present a set of test criteria based on our findings.


%To answer the question {\it which callback sequences are important to test}, we performed three studies. We classified the interactions between callbacks and designed a set of test criteria based on our findings.

%In this section we introduce new coverage criteria based on sequences of callbacks. We first present 3 studies to guide us on the designing of practical coverage criteria. Then, introduce how we model the execution of Android apps using callbacks. Finally, we present 3 coverage criteria based on callback sequences.

\subsection{Types of Callback Interactions}
%Android apps are mainly implemented by extending the Android API and writing callbacks which serve as main entry points of the app. Android apps are event and framework based. Their execution model is similar to previous GUI applications in which a main thread uses a message passing mechanism to handle all tasks posted by different external events (\eg GUI, GPS, etc.) and tasks posted by API calls made by the app. Each task is executed when it is removed from the event queue associated with the main thread. A task is executed atomically (no other task preempts the execution of the task) and can invoke one or more callbacks. 
To identify the types of callback interactions that exist in the apps, we need to understand how Android apps are executed. When an app is started, the Android system starts a process with one thread of execution (called main thread) \cite{processes}. All callbacks of the apps are executed in this thread by the framework. Similar to other event-driven systems, Android uses a message passing mechanism to handle the dispatching of events. This mechanism associates a message queue to the main thread and uses a \textit{Looper}\footnote{\url{https://developer.android.com/reference/android/os/Looper}} to dequeue the messages from the queue. After the Looper dequeues a message, it executes a task or action associated with the message. Each task is a method in the Android framework that can execute sequences of callbacks. For example, when an app is launched, the system posts a message to the main thread to execute the launch task for the app. This task is a method in the framework that executes the callbacks \inlinecode{onCreate()} $\to$ \inlinecode{onStart()} $\to$ \inlinecode{onResume()} for the main activity in the app. Besides external events, API methods can also send messages to the main thread. For example, the API method \inlinecode{Context.startService()} sends two messages to execute callbacks \inlinecode{onCreate()} and \inlinecode{onStartCommand()} for a service in the app. Callbacks can also invoke other callbacks synchronously through API methods \cite{DaniloMobile17}.  


\begin{table}[!ht]
	\centering
	\caption{Modeling Callback Interactions}\label{tab:controlparameters}
	%	\resizebox{\columnwidth}{!}{
	\begin{tabular}{|l||l|l|} \hline
		\textbf{Transfer of Control flow} & Follow & Callee
		\\\hline
		\textbf{Type of Execution} &	Synchronous & 	Asynchronous
		\\\hline
	\end{tabular}
%	}
\end{table}


In this paper, we model callback interactions by identifying how the control can change from one callback to another. Shown in Table~\ref{tab:controlparameters}, we used two parameters to describe such interactions.
The \textit{Transfer of Control Flow} parameter specifies whether the second callback is invoked after the first callback is accomplished, namely {\it follow}, or it is invoked by the first callback as a {\it callee} (the first callback uses an API method to invoke the second callback). The \textit{Type of Execution} parameter determines whether two callbacks are executed in the same task (\textit{Synchronous}) or different tasks (\textit{Asynchronous}) posted to the event queue.  Combining the two parameters, we can describe an interaction using a pair of \textit{(Transfer of Control Flow, Type of Execution)}. 
%When an app is run, the system creates a thread to handle all different external events (\eg GUI, GPS, etc.) and tasks posted by API calls made by the app. Android uses a single threaded message passing model in which each task posted to an event queue associated with the main thread can execute multiple callbacks \cite{processes}. We can model the execution of an Android app by identifying how the callbacks are invoked by the framework and their order. To define the possible interactions between callbacks, we need to understand how the control changes between callbacks. We identify the different ways in which the control can change from one callback to another using two main parameters shown in Table \ref{tab:controlparameters}. 

Based on Table~\ref{tab:controlparameters}, there can exist four types of interactions between two callbacks. The callbacks \textit{A} and \textit{B} have a relation \textit{(Synchronous, Follow)} when both callbacks are executed in the same task and the execution of \textit{B} follows after \textit{A}. As an example, the callbacks \inlinecode{onCreate} and \inlinecode{onStart} in activities are executed one after the other in the same task. In the case of \textit{(Asynchronous, Follow)}, a callback \textit{B} is executed also after \textit{A}, but \textit{B} is invoked asynchronously, and \textit{A} and \textit{B} are executed in different tasks. For example, two callbacks \textit{A} and \textit{B} that react to different GUI events are executed in different tasks; if  \textit{A} responses to an event happens before the event that {\textit B} handles, \textit{B} is put to the event queue during or after the execution of \textit{A}. In the third case, \textit{(Synchronous, Callee)} represents the scenario that during the execution of a callback \textit{A}, a callback \textit{B} is invoked synchronously by an API call. For example, in Figure \ref{fig:filedownloder610code} at line~5 the app calls the API method \inlinecode{getWritableDatabase()}. The API method synchronously invokes callbacks \inlinecode{DBHelper.onCreate()} or \inlinecode{DBHelper.onUpgrade()}. The change of control from \inlinecode{FDService.onCreate()} to \inlinecode{DBHelper.onUpgrade()} is categorized as \textit{(Synchronous,Invocation)} because the execution of \inlinecode{DBHelper.onUpgrade()} happens during the execution of \inlinecode{FDService.onCreate()} in the same task. Lastly, \textit{(Asynchronous, Callee)} describes the interaction that during the execution of callback \textit{A}, an API call schedules a task on the event queue which eventually executes a callback \textit{B}. For example, the API method \inlinecode{Handler.post} schedules a \inlinecode{Runnable} object on th event queue which eventually executes the callback \inlinecode{Runnable.run()}. 



\subsection{Studies of Callback Interactions}
To further understand what types of callback are important to test, we performed a set of studies. We designed our studies based on three intuitions. First, we believe that if there exists {\it valueflow} between two callbacks, we need to test the paths that traverse the inter-callback valueflow, as any mistakes and bugs related to the global valueflow may only be exposed through exercising inter-callback paths. For example, an object may be associated with a source and a sink that are located in different callbacks. To detect the bug where a source is missing or a sink is missing, we need to test the paths that traverse the callbacks. Second, we want to investigate whether there are callbacks frequently invoked together. If so, we need to test such callback sequences to ensure that the frequently occurred behaviors are tested. Third, we need to learn whether there exist bugs whose root causes are related to specific callback sequences. We need to especially test such interactions of callbacks to avoid similar bugs in different apps. In the following, we present our three studies based on the three intuitions respectively.

%The generation of all possible sequences of callbacks from the CCFA can be infinite. For finite applicability of a coverage criterion, we need to define the maximum number of callbacks in a callback sequence. 
%For the design of coverage criteria based on callbacks, we want to verify what types of callbacks (\eg callbacks related to GPS, GUI or camera events) are important to cover during testing. We present three studies: an empirical study to understand how data flows between callbacks, a trace analysis to identify common callback interactions, and a bug study. 
%we explore different bug patterns in Android apps and performed an empirical study to understand how data flows between callbacks. These two factors guide us to decide which callbacks should be covered and the length of the callback sequences. 

%First, we need to decide which types of callbacks should be covered. We want to verify whether. To identify the types of callbacks we categorized them based on their source of execution and whether they are executed asynchronously or not. The source of execution can be an external event (\eg a GUI event, a GPS location update or a tab to the power button) or an API call. All callbacks invoked in external events are invoked asynchronously whereas an API method can execute a callback synchronously or asynchronously (\eg the callback \inlinecode{onStartCommand} is executed asynchronously after calling \inlinecode{startService}). Thus, we have three categories of callbacks: \textit{ASYNC} (asynchronous callbacks executed from external events), \textit{API\_SYNC} (synchronous callbacks executed in API methods) and \textit{API\_ASYNC} (asynchronous callbacks executed in API methods). 

\paragraph{Study 1: callbacks involved in global valueflow.} 

In this study, we aim to answer:

{\bf RQ1:} does valueflow frequently occur between callbacks?

{\bf RQ2:} what types of callback interactions are involved in inter-callback valueflow?

We performed value flow analysis for all the variables  for the Android apps on 55 apps randomly selected from the Google Play Market\footnote{\url{https://play.google.com}}.  Our valueflow analysis indicates that 22.76\% of all source-sink pairs are located in different callbacks.  Analyzing inter-callback source-sink pairs, we found that 55\% source-sink pairs are located in callbacks that are not related to the API methods. There are 24\% of the inter-callback source-sink pairs that involve callbacks invoked synchronously in API methods (synchronous, follow), and 21\% that involve callbacks invoked asynchronously in API methods. 



%The flow of data between program variables has been shown to be an important metric to detect faults in certain programs \cite{dataflowtesting1, dataflowtesting2, databasedataflow}. We performed a valueflow analysis to determine the location of the definition of a value (source) and the location where the value is used (sink) on 55 apps which cover 20 out of 30 categories on the Google Play Market\footnote{\url{https://play.google.com}}. 

%To answer RQ2 for this study, we focus on analyzing \textit{inter-callback} source-sink pairs, where the source and sink are located in different callbacks. We study in what types of callbacks the source and sinks are located, meaning what types of callbacks share data. We classify the callbacks depending on the type interactions they can have. For example, if a callback is invoked by an API method, then the interaction is either \textit{(Synchronous, Invocation)} or \textit{(Asynchronous, Invocation)} depending on whether the callback is invoked synchronously or asynchronously. If the callback is a event listener for an external event, then it is categorized as \textit{(Asynchronous, Follows)} because these callbacks are always executed in their own tasks. For each inter-callback source-sink pair, we identify the interactions in which the source callback can be executed and the interactions in which the sink callback can be executed. Based on the set of those interactions, we determine whether C1, C2 or C3 will consider the execution of the callbacks interactions that represent the source-sink pair. 

%{\bf RQ1:} We found that 22.76\% of all source-sink pairs were inter-callbacks and that all apps in the study contain inter-callbacks source-sink pairs. This shows that the callbacks frequently share data in apps. 


{\bf RQ2:} what coverage criteria is needed to inter-callback valueflow?

The flow of data between program variables has been shown to be an important metric to detect faults in certain programs \cite{dataflowtesting1, dataflowtesting2, databasedataflow}. 
We performed a valueflow analysis to determine the location of the definition of a value (source) and the location where the value is used (sink) on 55 apps which cover 20 out of 30 categories on the Google Play Market\footnote{\url{https://play.google.com}}. 

To answer RQ2 for this study, we focus on analyzing \textit{inter-callback} source-sink pairs, where the source and sink are located in different callbacks. We study in what types of callbacks the source and sinks are located, meaning what types of callbacks share data. We classify the callbacks depending on the type interactions they can have. For example, if a callback is invoked by an API method, then the interaction is either \textit{(Synchronous, Invocation)} or \textit{(Asynchronous, Invocation)} depending on whether the callback is invoked synchronously or asynchronously. If the callback is a event listener for an external event, then it is categorized as \textit{(Asynchronous, Follows)} because these callbacks are always executed in their own tasks. For each inter-callback source-sink pair, we identify the interactions in which the source callback can be executed and the interactions in which the sink callback can be executed. Based on the set of those interactions, we determine whether C1, C2 or C3 will consider the execution of the callbacks interactions that represent the source-sink pair. 

{\bf RQ1:} We found that 22.76\% of all source-sink pairs were inter-callbacks and that all apps in the study contain inter-callbacks source-sink pairs. This shows that the callbacks frequently share data in apps. 

{\bf RQ2:} Table \ref{tab:sourcesinkresults} shows the results of the study. More than a half of the source-sink pairs (55\%) are present in callbacks that are not related to API methods. The interactions of these callbacks can be covered by C1. There are 24\% of the inter-callback source-sink pairs that involve callbacks invoked synchronously in API methods and 21\% that involve callbacks invoked asynchronously in API methods. 

\begin{table}[ht!]
	\centering
	\caption{Percentage of Source-Sink Pairs Covered}\label{tab:sourcesinkresults}
	%	\resizebox{\columnwidth}{!}{
	\begin{tabular}{|l|l|} \hline
		Coverage Criterion & Source-Sink Pairs Covered  \\ \hline  \hline
		C1 & 55\% \\ \hline
		C2 & 79\% \\ \hline
		C3 & 100\%  \\ \hline
	\end{tabular}
	%	}
\end{table}
>>>>>>> 29fbe5cd55c1fe5b8ef388520bb3671e84cdf5a1
% We define two categories for callbacks: callbacks invoked in external events (\eg GUI, GPS and sensors) or windows (Activities, Menus or Dialogs) and callbacks invoked in API methods (\eg in Figure \ref{fig:filedownloder610code} the callback \inlinecode{DBHelper.onUpgrade()} is invoked in the API method \inlinecode{getWritableDatabase()}). The execution of the first category of callbacks can be captured by the callback interactions \textit{(Synchronous, Follows)} and \textit{(Asynchronous, Follows)}. For the second category,
%We study two main aspects of these inter-callback source-sink pairs. The first aspect is the type of callbacks in which the sources and sinks are located. The second aspect is the number of callbacks that a source has to transition in the CCFA to reach a sink. We identify two kind of callbacks: callbacks invoked from external events and callbacks invoked in API calls. We use this information to decide whether 

%To identify the types of callbacks we categorized them based on their source of execution and whether they are executed asynchronously or not. The source of execution can be an external event (\eg a GUI event, a GPS location update or a tab to the power button) or an API call. All callbacks invoked in external events are invoked asynchronously whereas an API method can execute a callback synchronously or asynchronously. Thus, we have three categories of callbacks: \textit{ASYNC} (asynchronous callbacks executed from external events), \textit{API\_SYNC} (synchronous callbacks executed in API methods) and \textit{API\_ASYNC} (asynchronous callbacks executed in API methods). 

%We found that the inter-callback source-sink pairs are present in all apps, meaning that the data sharing between callbacks is common in apps. Our results show that the value flows between callbacks executed from external events or windows account for 55\% of all the value flows found in the study and value flows between callbacks invoked in API methods account for the 34\% of flows. Value flows between callbacks invoked in external events and callbacks invoked in API methods account for 16\%. We found that most of the source-sink pairs (35\%) take just one callback to reach the sink. Thus, a coverage criterion based on just sequences of callbacks invoked in external events or windows should be considered since most of the data shared between callbacks is made on those types of callbacks. 

%We also studied the number of callbacks it takes a source to reach a sink in the CCFA (if the next callback from a source in the CCFA contains the sink, then we say that the length is 1). We found that most of the source-sink pairs take just one callback (34\%). The maximum length we observed was 18 (less than 1\%) and the median was 3. Therefore, sequences containing 2 (length 1) to 4 callbacks (length 3) are the most frequent length of callbacks between a source and sink. 


\paragraph{Study 2: frequent callback sequences in traces.} In this study, we aim to answer:


{\bf RQ1:} what callback interactions frequently occur in traces?
%{\bf RQ1:} does certain callbacks frequently occur together in traces?

%{\bf RQ2:} if so, what types of callbacks are they? are they app-specific?


To identify what sequences of callbacks are most common in apps, we instrumented 5 apps (\textit{ContactsList}, \textit{StandupTimer}, \textit{BARIA}, \textit{JustCraigslist} and \textit{OpenSudoku}) and collected traces by testing the apps manually. We then mine the most common sequences with two callbacks considering the type of callback. We use the CCFA representation \cite{DaniloTSE19} to categorize each interaction found in the traces. 

{\bf RQ1:} We found that from that 64\% of the callbacks interactions are either \textit{(Synchronous, Follows)} or \textit{(Asynchronous, Follows)}. The rest of the interactions found in the traces account for 21\% \textit{(Synchronous, Invocation)} and 15\% \textit{(Asynchronous, Invocation)}. Similarly to the first study, the callback interactions \textit{(Synchronous, Follows)} and \textit{(Asynchronous, Follows)} dominate the behavior in the traces. 

%contain just callbacks invoked in API methods. Sequences containing a mix with callbacks invoked in external events or windows and callbacks invoked API methods account for the 15\%. This is a similar pattern to what we found in the previous study, implying that the most of the data shared and most of the interactions of callbacks is between callbacks invoked in external events and windows. Therefore, a coverage criterion should cover these behaviors. 

%The races observed in Android apps most commonly occur between ASYNC callbacks and between ASYNC and API\_ASYNC callbacks \cite{cgeo3991}. The example shown in Figures \ref{fig:chanu140code} and \ref{fig:chanu140subseq} show a data race between ASYNC callbacks (from callbacks that react to GUI and camera events). Concurrency faults between ASYNC and API\_ASYNC callbacks are also common. For example, in the issue \#3991 for the app \textit{cgeo}~\cite{cgeo3991}, there is data race condition between a tab to the back button (execute ASYNC callbacks) and an asynchronous callback executed using the API method \inlinecode{Handler.sendMessage}.   One of the challenges to generate sequences of callbacks from the CCFA that contain API\_ASYNC callbacks is that the CCFA keeps the order in which the API\_ASYNC callbacks are added to the event-queue but not all the possible executions at runtime. Therefore, the generated callback sequences cannot be directly compared against dynamic traces. We introduce the parameter \textit{Follows Immediately} to determine whether we can compute all the callback sequences directly from the CCFA or not. 

\paragraph{Study 3: pairs of callbacks that lead to bugs.}

In this study, we aim to answer:


{\bf RQ1:} how often are the {\it inter-callback bugs} (bugs whose root causes are related to more than one callback) reported?

%{\bf RQ2:}  what types of callbacks are relevant to the inter-callback bugs?
{\bf RQ2:}  what callback interactions are relevant to the inter-callback bugs?
<<<<<<< HEAD

We performed a bug study on 6 open source apps. We focus on bugs in which the root cause is related the interaction of callbacks (a certain callback path created a condition that crashed the app). Our methodology was to focus on crashes in the apps. We filter all the closed bugs by using the following keywords: crash, NPE, exception and runtime exception. Then, we manually inspected the bugs to determine the root cause. If the root cause involve a particular callback interaction, then we identify the set of callback interactions needed to trigger the bug. Table \ref{tab:bugstudy} shows the results of the study. Note that if the bug requires callback interactions \textit{(Asynchronous, Follows)} and \textit{(Synchronous,Follows)} we categorize it as the behavior to trigger the bug can be cover by C1. If the bug includes an \textit{(Synchronous, Invocation)} interaction, then we categorize it as C2. Lastly, if the bug includes an \textit{(Asynchronous, Invocation)}, the behavior can only be covered by C3. 

\begin{table}[!ht]
	\centering
	\caption{Bug Study Results}\label{tab:bugstudy}
%	\resizebox{\columnwidth}{!}{
		\begin{tabular}{|l|r|r|r|r|} \hline
			App & Bugs & C1 & C2 & C3 \\ \hline \hline
			ConnectBot & 9 & 0 & 0 & 4 \\ \hline
			FileDownloader & 12 & 0 & 1 & 1 \\ \hline
			AntennaPod & 133 & x & 0 & 5 \\ \hline
			cgeo & 273 & x & 0 & 4 \\ \hline
			Wordpress & 315  & x & 2 & 2 \\ \hline
			Ankidroid & 784  & x & 1 & 4 \\ \hline
			\textbf{Total} & \textbf{1526} & \textbf{x} &  \textbf{4} & \textbf{20} \\ \hline
		\end{tabular}
%	}
\end{table}

{\bf RQ1:} Inter-callback bugs were frequent among all apps. We found a total of 24 bugs related to inter-callbacks apps in 1526 bugs studied. 

{\bf RQ2:} The most relevant interactions were \textit{(Asynchronous, Invocation)}. We see that the main cause of these bugs is the lack of knowledge of all possible callback paths that can be executed when there are other asynchronous callbacks. 

\paragraph{Conclusions of the Studies} In studies 1 and 2 we found that the most of the data is shared between callbacks and the callback interactions involve callbacks invoked in external events or windows (modeled by interactions \textit{(Synchronous, Follows)} and \textit{(Asynchronous, Follows)}). This tells us that the majority of the app implementation is related to GUI (including windows and GUI event handlers) and external events related to components of the phone such as GPS, camera, etc. However, our bug study shows that the callbacks invoke in API methods are prompt to introduce faults. Coverage criterion C1 can be a useful metric for test suites of certain apps that rely mostly on GUI and external events. On the other hand, for bigger and more complex apps, C2 and C3 can be more efficient metrics.
%We explore different bug patterns that are not covered by current event-based and structural coverage criteria. The first bug pattern we evaluate is related to the execution of asynchronous callbacks. Asynchronous callbacks can be executed from different external events (\eg GUI, network and sensors) and also from API calls (\eg \inlinecode{Handler.sendMessage} and \inlinecode{Context.startService}). This can create data races due to different interleaving of callbacks \cite{raceandroidmaiya, raceandroidhsiao, racebielik}. Sequences of methods (specially pair of methods) have been used before for coverage criteria designed to detect concurrency bugs \cite{choudharyconcurrency, tasharoficoncurrency}. Thus, we consider that callback sequences are an adequate metric to cover concurrency faults in Android apps. 
%
%The races observed in Android apps most commonly occur between callbacks with a relation \textit{(Asynchronous, Follows)} \cite{raceandroidmaiya, raceandroidhsiao}. The example shown in Figures \ref{fig:chanu140code} and \ref{fig:chanu140subseq} show a data race between callbacks of two different external events (callbacks that react to GUI and camera events). Concurrency faults between callbacks from external events and asynchronous callbacks invoked in API calls are also frequent. For example, in the issue \#3991 for the app \textit{cgeo}~\cite{cgeo3991}, there is data race condition between a tab to the back button and an asynchronous callback executed using the API method \inlinecode{Handler.sendMessage}. Thus, the asynchronous interactions between external events (not just GUI events) and also between callbacks invoke in API calls are important to cover. 
%
%Another bug pattern we study is related to the different behaviors that an API call can have with respect of the sequences of callback it executes. Figures \ref{fig:filedownloder610code} and \ref{fig:filedownloader610subseq} shows an example of this bug pattern. In Figure \ref{fig:filedownloader610subseq} we see that there are interactions \textit{(Synchronous, Invocation)}. We design a coverage criterion with this kind of interactions to evaluate how important they are in fault detection. 
\subsection{Designing Testing Criteria Based on Callback Interactions}
We have identified four types of callback interactions based on the control change between two callbacks. We have used examples to show these interactions are feasible. In this section, we develop three testing criteria, namely {\it C1}, {\it C2} and {\it C3}, that aim to cover these interactions. Shown in Table \ref{tab:coveragecriteria}, the criteria is designed in a way that {\it C1} is the weakest, {\it C2} is stronger by including one more type of interaction, and {\it C3} is the strongest that aim for covering all types of the interactions. In the following, we further show that there are different sets of app behaviors that can be covered by C1, C2 and C3. 

%The main hypothesis of this paper is that current GUI event-based and structural coverage criteria are not the best metrics to verify the adequacy of a test suite. We want to test the hypothesis that a more specialized coverage criteria is needed besides GUI event-based ones. We design 3 coverage criteria, one more complex than the other to observe whether the behaviors added are important to identify faults. Each coverage criterion is defined based on the type of callbacks interactions they cover. Table \ref{tab:coveragecriteria} shows the 3 different coverage criteria we define and the callbacks interaction that each of them cover. 

%Each coverage criterion is defined based on type of interactions they cover. 

%Therefore, by covering just certain changes of control between callbacks, a coverage criterion focus on specific behaviors in the app. Table \ref{tab:coveragecriteria} shows 4 coverage criteria we define. 


\begin{table}
	\centering
	\caption{Testing Criteria based on Callback Interactions}\label{tab:coveragecriteria}
	%	\resizebox{\columnwidth}{!}{
	\begin{tabular}{|l|l|} \hline
		Name & Covered Callback Interactions  \\ \hline  \hline
		C1 & \textit{(Asynchronous,Follow)}, \textit{(Synchronous,Follow)} \\ \hline
		C2 & C1 $+$ \textit{(Synchronous, Callee)} \\ \hline
		C3 & C2 $+$ \textit{(Asynchronous, Callee)}  \\ \hline
	\end{tabular}
	%	}
\end{table}

%\paragraph{Coverage Criterion C1.} 
{\it C1} aims to cover the callback interactions \textit{(Asynchronous, Follow)} and \textit{(Synchronous, Follow)}. which means it does not consider any callback invoked, synchronously or asynchronously, in API methods. The behaviors covered by C1 are close to the behaviors of a GUI model. The difference with a coverage criterion based on GUI callbacks is that C1 also requires to exercise the behaviors between callbacks invoked in other kind of external events besides GUI events. For example, if an app registers a listener to receive location updates from the GPS, C1 covers any interaction between the location listener callbacks and any other callback that is executed in a different asynchronous task (\eg GUI event callback listener). To satisfy C1, the testing needs to consider generating external events besides GUI events in order to trigger all the possible callback interactions found in the app. % As we have seen in previous studies \cite{stoat}, the generation of external events, besides GUI events, is important to trigger certain kind of bugs. 

%\paragraph{Coverage Criterion C2}
C2 adds the set of callback interactions \textit{(Synchronous, Invocation)} on top of C1. These interactions are related to callbacks that are invoked synchronously in API methods. As shown in Section \ref{sec:motivation}, API methods can execute different sequences of callbacks when executed under different environments. The bug can be missed if testing does not sufficiently cover different paths of the relevant part of the framework, triggered by different environments.

C2 adds the set of callback interactions \textit{(Synchronous, Invocation)} on top of C1. The advantage of considering \textit{(Synchronous, Invocation)} interactions if a test suite misses the execution of an API call that invokes callbacks synchronously, it will be reflected in all the callback interactions the API method executes. However, an event-based coverage criteria, would not have knowledge about these execution paths. Even when a test suite reaches an API call that invokes callbacks synchronously, there are some cases in which the API method can execute different callbacks under different states of the system. As we presented in the example showed in Figures \ref{fig:filedownloder610code} and \ref{fig:filedownloader610subseq}, for some API methods, the app needs certain state to trigger all the possible callbacks invoked in a method (in this case, an older app already installed in the system). Another example can be seen in the API method \inlinecode{LoaderManager.initLoader()}. This method will the execute callback \inlinecode{LoaderCallbacks.onCreateLoader()} if the data the loader has not been created or \inlinecode{LoaderCallbacks.onLoad()} if the loader has been created and data was already loaded. Thus, the different callbacks interactions in an API method, provide knowledge about the different paths that need to be cover in the framework.




%which means that the environment can help to increase the branch coverage on the framework code.  To satisfy C2, test suites have to test the apps under the environments that can cover different paths of the framework. C2 might add just few behaviors depending on the how the app is implemented, but these behaviors might be important on detecting whether the app has bugs or not.

%\paragraph{Coverage Criterion C3}
C3 adds the set of callbacks interactions \textit{(Asynchronous, Invocation)} on top of C2. \textit{(Asynchronous, Invocation)} callback interactions are harder to reason about for the developer because the there are multiple order of execution of this callbacks with respect to all the other asynchronous callbacks. Test suites that satisfy C3 must exercise the concurrent behavior that an app can present from not just external events, but the interaction of external events and callbacks invoked asynchronously in API methods. 

C3 adds the set of callbacks interactions \textit{(Asynchronous, Invocation)} on top of C2. C3 is designed to cover asynchronous between asynchronous callbacks invoked in API calls (\eg \inlinecode{Handler.sendMessage} and \inlinecode{Context.startService}) and also asynchronous callbacks invoked in external events. Concurrency faults related to asynchronous callbacks invoked in API calls have been studied before \cite{raceandroidmaiya, raceandroidhsiao, racebielik}. They can be frequent in apps that include several asynchronous callbacks. For example, in the issue \#3991 for the app \textit{cgeo}~\cite{cgeo3991}, there is data race condition between a tab to the back button and an asynchronous callback executed using the API method \inlinecode{Handler.sendMessage}. Thus, the asynchronous interactions between external events (not just GUI events) and also between callbacks invoke in API calls are important to cover.

Sequences of methods (specially pair of methods) have been used before for coverage criteria designed to detect concurrency bugs \cite{choudharyconcurrency, tasharoficoncurrency}. Thus, we consider that callback interactions in C3 are an adequate metric to cover concurrency faults in Android apps. Test suites that satisfy C3 must exercise the concurrent behavior that an app can present from not just external events, but the interaction of external events and callbacks invoked asynchronously in API methods 


=======

We performed a bug study on 6 open source apps. We focus on bugs in which the root cause is related the interaction of callbacks (a certain callback path created a condition that crashed the app). Our methodology was to focus on crashes in the apps. We filter all the closed bugs by using the following keywords: crash, NPE, exception and runtime exception. Then, we manually inspected the bugs to determine the root cause. If the root cause involve a particular callback interaction, then we identify the set of callback interactions needed to trigger the bug. Table \ref{tab:bugstudy} shows the results of the study. Note that if the bug requires callback interactions \textit{(Asynchronous, Follows)} and \textit{(Synchronous,Follows)} we categorize it as the behavior to trigger the bug can be cover by C1. If the bug includes an \textit{(Synchronous, Invocation)} interaction, then we categorize it as C2. Lastly, if the bug includes an \textit{(Asynchronous, Invocation)}, the behavior can only be covered by C3. 

\begin{table}[!ht]
	\centering
	\caption{Bug Study Results}\label{tab:bugstudy}
%	\resizebox{\columnwidth}{!}{
		\begin{tabular}{|l|r|r|r|r|} \hline
			App & Bugs & C1 & C2 & C3 \\ \hline \hline
			ConnectBot & 9 & 0 & 0 & 4 \\ \hline
			FileDownloader & 12 & 0 & 1 & 1 \\ \hline
			AntennaPod & 133 & x & 0 & 5 \\ \hline
			cgeo & 273 & x & 0 & 4 \\ \hline
			Wordpress & 315  & x & 2 & 2 \\ \hline
			Ankidroid & 784  & x & 1 & 4 \\ \hline
			\textbf{Total} & \textbf{1526} & \textbf{x} &  \textbf{4} & \textbf{20} \\ \hline
		\end{tabular}
%	}
\end{table}

{\bf RQ1:} Inter-callback bugs were frequent among all apps. We found a total of 24 bugs related to inter-callbacks apps in 1526 bugs studied. 

{\bf RQ2:} The most relevant interactions were \textit{(Asynchronous, Invocation)}. We see that the main cause of these bugs is the lack of knowledge of all possible callback paths that can be executed when there are other asynchronous callbacks. 

\paragraph{Conclusions of the Studies} In studies 1 and 2 we found that the most of the data is shared between callbacks and the callback interactions involve callbacks invoked in external events or windows (modeled by interactions \textit{(Synchronous, Follows)} and \textit{(Asynchronous, Follows)}). This tells us that the majority of the app implementation is related to GUI (including windows and GUI event handlers) and external events related to components of the phone such as GPS, camera, etc. However, our bug study shows that the callbacks invoke in API methods are prompt to introduce faults. Coverage criterion C1 can be a useful metric for test suites of certain apps that rely mostly on GUI and external events. On the other hand, for bigger and more complex apps, C2 and C3 can be more efficient metrics.
%We explore different bug patterns that are not covered by current event-based and structural coverage criteria. The first bug pattern we evaluate is related to the execution of asynchronous callbacks. Asynchronous callbacks can be executed from different external events (\eg GUI, network and sensors) and also from API calls (\eg \inlinecode{Handler.sendMessage} and \inlinecode{Context.startService}). This can create data races due to different interleaving of callbacks \cite{raceandroidmaiya, raceandroidhsiao, racebielik}. Sequences of methods (specially pair of methods) have been used before for coverage criteria designed to detect concurrency bugs \cite{choudharyconcurrency, tasharoficoncurrency}. Thus, we consider that callback sequences are an adequate metric to cover concurrency faults in Android apps. 
%
%The races observed in Android apps most commonly occur between callbacks with a relation \textit{(Asynchronous, Follows)} \cite{raceandroidmaiya, raceandroidhsiao}. The example shown in Figures \ref{fig:chanu140code} and \ref{fig:chanu140subseq} show a data race between callbacks of two different external events (callbacks that react to GUI and camera events). Concurrency faults between callbacks from external events and asynchronous callbacks invoked in API calls are also frequent. For example, in the issue \#3991 for the app \textit{cgeo}~\cite{cgeo3991}, there is data race condition between a tab to the back button and an asynchronous callback executed using the API method \inlinecode{Handler.sendMessage}. Thus, the asynchronous interactions between external events (not just GUI events) and also between callbacks invoke in API calls are important to cover. 
%
%Another bug pattern we study is related to the different behaviors that an API call can have with respect of the sequences of callback it executes. Figures \ref{fig:filedownloder610code} and \ref{fig:filedownloader610subseq} shows an example of this bug pattern. In Figure \ref{fig:filedownloader610subseq} we see that there are interactions \textit{(Synchronous, Invocation)}. We design a coverage criterion with this kind of interactions to evaluate how important they are in fault detection. 
>>>>>>> 29fbe5cd55c1fe5b8ef388520bb3671e84cdf5a1



==> discussion.tex <==
\section{Discussions}
We only consider length of 2 interactions, we can extend it to n; we only consider immediately follow, callee,  but can be extend to add space between the two callbacks 

==> evaluation.tex <==
\section{Evaluation}
The main focus of our evaluation is to verify coverage criteria based on callback sequences. Thus, we focus on answering the following research questions:

\noindent \textbf{RQ1. Possible Behaviors.} Is the number of possible behaviors (or callback sequences) that need to be satisfied different for callback-based coverage criteria greater than a coverage criterion based just on GUI behavior? 


\noindent \textbf{RQ3. Tests Effectiveness.} 


\subsection{Evaluation Setup}
We compare the coverage of C1, C2 and C3 against statement coverage and GUI coverage. To measure statement coverage, we built the app with instrumentation support using Jacoco \cite{jacoco}. To measure GUI coverage, we compute sequence of callbacks using the approach for computing C1 but without considering EVENT callbacks that do not react to GUI events (\eg GPS location update or sensors callbacks). We generate sequences involving two callbacks as well as in C1. 

We evaluate our coverage criteria on 10 randomly selected apps from the open source repository F-droid \cite{fdroid} and chanu to test our motivating example. Table \ref{tab:benchmarks} presents the benchmarks we selected with their category, total lines of source code (column SLOC), and the time that Monkey was run to test the app. 



\begin{table}[!ht]
	\centering
	\caption{Benchmarks}\label{tab:benchmarks}
	\resizebox{\columnwidth}{!}{
	\begin{tabular}{|l|l|r|r|} \hline
		App & Category & SLOC & Test Time (min) \\ \hline \hline
		Location Share & Navigation & 384 & 60 \\ \hline
		Calculator & Tools & 629 & 30 \\ \hline
		Pushup Buddy & Health \& Fitness & 965 & 60 \\ \hline
		SdbViewer & Tools & 1273 & 180 \\ \hline
		Cache Cleaner & Tools & 1493 & 180 \\ \hline
		Movie DB & Entertainment & 4727 & 180 \\ \hline
		BART Runner & Navigation & 6124 & 180 \\ \hline
		Open Sudoku & Games & 6440 & 180 \\ \hline
		Mileage & Finance & 9931 & 180 \\ \hline
		Pedometer & Health \& Fitness & 13502 & 180\\ \hline
		chanu & Social & 45856 & 180 \\ \hline
	\end{tabular}
		}
\end{table}


\subsection{RQ1. Possible Behaviors}
We compare the behaviors of each coverage criteria C1, C2 and C3 against GUI coverage and statement coverage and study. Table \ref{tab:sequences} shows the coverage for C1, C2, C3, GUI and statements for all the benchmarks. For C1, C2, C3 and GUI we present the total number of sequences covered by the tests (column C), the total number of sequences (column T), and the percentage of coverage. 

\begin{table*}[!ht]
	\centering
	\caption{Coverage for C1, C2, C3, GUI and Statement Coverage}\label{tab:sequences}
	%\resizebox{\columnwidth}{!}{
	\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|} \hline
		\multirow{2}{*}{App} & \multicolumn{5}{|c|}{Manual} & \multicolumn{5}{|c|}{Monkey} & \multicolumn{5}{|c|}{Stoat} \\ \cline{2-16}
		& C1 & C2 & C3 & GUI & Stmt & C1 & C2 & C3 & GUI & Stmt & C1 & C2 & C3 & GUI & Stmt \\
		 \hline
		Location Share & 51\% & - & - & 72\% & 90.6\% & 33\% & - & - & 62\% & 65\% & x & - & - & x & x \\ \hline
		Calculator & 35.08\% & - & - & 35.08\% & 65.98\% & 95.98\% & - & - & 95.98\% & 85.93\% & x & - & - & x & x \\ \hline 
	\end{tabular}
\end{table*}

\begin{table*}[!ht]
	\centering
	\caption{Coverage for C1, C2, C3, GUI and Statement Coverage}\label{tab:sequences}
	%\resizebox{\columnwidth}{!}{
		\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|} \hline
			\multirow{2}{*}{App} & \multicolumn{3}{|c|}{C1} & \multicolumn{3}{|c|}{C2} & \multicolumn{3}{|c|}{C3} & \multicolumn{3}{|c|}{GUI} & \multirow{2}{*}{Stmt (\%)}  \\ \cline{2-13}
			& C & T & \% & C & T  & \% & C & T  & \% & C & T  & \% &  \\ \hline \hline
			Location Share & 73 & 154 & 47.40 & - & - & - & - & - & - & 45 & 62 & 72.58 & 90.89  \\ \hline
			Calculator & 1834 & 1923 & 95.37 & - & - & - & - & - & - & 1834 & 1923 & 95.37 & 85.93 \\ \hline
			Pushup Buddy & 116 & 272 & 42.64 & 16 & 122 & 13.11 & 15 & 36 & 41.67 & 92 & 230 & 40.00 & 90.89  \\ \hline
			SdbViewer & 90 & 188 & 47.87 & - & - & - & 6 & 24 & 25.00 & 29 & 42 & 69.05 & 90.89  \\ \hline
			Cache Cleaner & 11 & 25 & 44 & 6 & 10 & 60 & 10 & 14 & 71.43 & 11 & 25 & 44.00 & 71.92  \\ \hline
			Movie DB & 58 & 163 & 35.58 & 12 & 44 & 27.27 & 64 & 182 & 35.16 & 52 & 135 & 38.51 & 41.61 \\ \hline
			BART Runner & 154 & 563 & 27.35 & - & - & - & 261 & 506 & 51.58 & 51 & 192 & 26.56 & 65.89 \\ \hline
			Open Sudoku & 69 & 280 & 24.64 & 8 & 110 & 0.73 & 17 & 54 & 31.48 & 69 & 280 & 24.64 & 59.87 \\ \hline
			Mileage & 203 & 861 & 23.58 & 15 & 43 & 34.89 & 12 & 55 & 21.82 & 203 & 861 & 23.58 & 50.89 \\ \hline
			Pedometer & 68 & 106 & 64.15 & 6 & 27 & 22.22 & 167 & 212 & 78.77 & 68 & 106 & 64.15 & 77.75 \\ \hline
			chanu & 204 & 576 & 35.42 & 59 & 206 & 28.64 & 173 & 359 & 48.19 & 200 & 567 & 35.27 & 59.57 \\ \hline
		\end{tabular}
%	}
\end{table*}

\paragraph{Behaviors in C1}
When comparing the number of behaviors in C1 compared to GUI, we observed that the 6 out of 10 apps have similar functionality since the number of sequences do not differ by a big number. That is because more of the EVENT callbacks in these apps are GUI callbacks. The apps with significant difference between C1 and GUI are Location Share, Pushup Buddy, SdbViewer, Movie DB and BART Runner. We study the sequences not covered in these apps and found that there are some behaviors that a tool such as Monkey is not able to test. For example, in Location Share we found there are valid sequences containing the callback \inlinecode{LocationListener.onStatusChanged} that were not covered by the tests. This callback is executed when the GPS signal is lost or found. Our tests were not run on an environment where the GPS signal was unstable which might covered more valid sequences. Similarly, Pushup Buddy uses \textit{Sensors}~\cite{sensors} to measure the motion of a push up exercise by the user. To improve the C1 coverage in these apps, we need tests that simulates environments generated by mobility (\eg flaky Internet connection or GPS signal). 

\paragraph{Behaviors in C2}

\subsection{RQ2. Tests Effectiveness.}
Table \ref{tab:faults} shows the faults found per app including total crashes during test and the unique crashes. To identify unique crashes, we focus on exceptions for the app (using the process name) and use the exception stack as identifier of the fault. We study in detail each app and the kind of faults that our tests were able to trigger. 

\begin{table}[!ht]
	\centering
	\caption{Benchmarks}\label{tab:faults}
%	\resizebox{\columnwidth}{!}{
		\begin{tabular}{|l|r|r|} \hline
			App & Total Crashes & Unique Crashes \\ \hline \hline
			Calculator & 169 & 4 \\ \hline
			Movie DB & 14 & 2 \\ \hline
			BART Runner & 3 & 3 \\ \hline
			Mileage & 123 & 2 \\ \hline
			Pedometer & 2 & 2 \\ \hline
			chanu & 4 & 3 \\ \hline
		\end{tabular}
%	}
\end{table}

\subsubsection{Calculator}


==> study.tex <==
\section{Callback-Based Coverage Criteria}
In this section we introduce new coverage criteria based on sequences of callbacks. We first introduce a representation to model the execution of Android apps using callbacks. Then, we performed three studies to understand how important to cover these interactions during testing. We finally present a set of test criteria based on our findings.

\subsection{Modeling the Android Apps using Callbacks}
Event-based, framework-based mobile apps base their implementation on callbacks provided by the Android framework's API. When an app is run, the framework will execute callbacks depending on external events and API calls made by the app. To model the execution of these callbacks, we consider 4 different changes of control between callbacks: 1) a callback $\mathit{B}$ is invoked synchronously after another callback $\mathit{A}$, 2) $\mathit{B}$ is invoked asynchronously after $\mathit{A}$, meaning $\mathit{B}$ is put in the event queue and invoked eventually after $\mathit{A}$ is invoked, 3) during an execution of $\mathit{A}$, $\mathit{B}$ is invoked synchronously by an API call, and 4) during an execution of $\mathit{A}$, $\mathit{B}$ is invoked asynchronously by an API call, meaning the API call puts $\mathit{B}$ in the event queue and the callback is invoked eventually after $\mathit{A}$. 

In order to compute the possible sequences of callbacks generated from the 4 different changes of control between callbacks, we use a static model called \textit{Callback Control Flow Automata} (CCFA) \cite{DaniloTSE19}. A CCFA is a representation based on the \textit{Extended Finite State Machine} (EFMS) \cite{1600197}. In CCFAs, transitions from one state to another represent transfer of control between callbacks. Each state represents whether the execution enters or exits a callback. Each transition can have a guard, which is a condition that enables the transition (decides whether the transition can be taken or not). These conditions can be external events (the execution of an event handler callback cannot be executed unless a GUI event is trigger) or API calls (the execution of a callback is made by an API method). The inputs of the CCFAs represent the entry and exit points of callbacks. We use $\mathit{callbackname_{entry}}$ and $\mathit{callbackname_{exit}}$ as input symbols so we can specify the case where one callback is invoked during the execution of the other (see Type 3 and Type 4 of control flow discussed above).

\figref{examplecode} shows an simple Android app with its respective CCFA in \figref{ccfa}. The CCFA shows a change of control from \inlinecode{A.onCreate()} to \inlinecode{A.onStart()} of type 1. Then, the transitions from $q_4$ to $q_6$ show a change of control from callback \inlinecode{A.onStart()} to \inlinecode{L.onCreateLoader()} of type 3. Note that the transition from the state $q_6$ to $q_7$ is guarded by a condition that checks whether the API call to \inlinecode{initLoader()} (at line 11 in \figref{examplecode}) was executed. Similarly, the transition from $q_5$ to $q_{10}$ is guarded by the execution of an event is represents a change of control of type 2. 

\begin{figure}
	\centering
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\resizebox{0.85\columnwidth}{!}{
			%\lstset{basicstyle=\listingsfont, numbers=left, language=Java}
			\lstinputlisting{code/example2.java}
		}
		\caption{Source code of a simple Android app\label{fig:examplecode}}        
	\end{subfigure}
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\resizebox{\columnwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.3cm,
			semithick]
			%\tikzstyle{every state}=[fill=cadmiumgreen,draw=none,text=white]
			
			\node[initial,state, accepting] (Q1)                    {$q_1$};
			\node[state]         (Q2)  [above right=of Q1, xshift=-0.6cm] {$q_2$};
			\node[state]         (Q3)  [right of=Q2] {$q_3$};
			\node[state]         (Q4)  [right of=Q3] {$q_4$};
			\node[state]         (Q5)  [below of=Q3,xshift=0.7cm] {$q_5$};
			\node[state]         (Q6)  [right of=Q4] {$q_6$};
			%            \node[state]         (Q7)  [below of=Q4] {$q_7$};
			\node[state]         (Q8)  [below of=Q6] {$q_7$};
			\node[state]         (Q9)  [below of=Q8] {$q_{8}$};
			\node[state]         (Q10) [left of=Q9, xshift=-0.6cm] {$q_{9}$};
			\node[state]         (Q11) [below of=Q2, xshift=-0.7cm] {$q_{10}$};
			\node[state]         (Q12) [below of=Q5] {$q_{11}$};
			%    \node[state,accepting,double]         (J) [right of=I]       {$q_{10}$};
			
			\path
			(Q1) edge[edgeasync]         node[align=center] {($\mathit{A.onCeate_{entry}}$, \\  $\mathit{evt = launch}$)} (Q2)
			(Q2) edge          node[align=center] {($\mathit{A.onCreate_{exit}}$, \\ $\mathit{true}$)} (Q3)
			(Q3) edge          node[align=center] {($\mathit{A.onStart_{entry}}$, \\ $\mathit{true}$)} (Q4)
			(Q4) edge         node[align=right, near end] {($\mathit{A.onStart_{exit}}$, \\ $\mathit{true}$)} (Q5)
			edge          node[align=center] {$\epsilon$} (Q6)
			%(Q6) edge          node[align=center, left, near start] {($L.onCreateLoader_{entry}$, \\  TRUE)} (Q7)
			(Q6) edge          node[align=center,left, near start] {\footnotesize ($\mathit{L.onCreateLoader_{entry}}$, \\ \footnotesize $\mathit{cs=lm.initLoader()}$)} (Q8)
			
			%    (Q7) edge          node[align=right, left, near start] {($L.onCreateLoader_{exit}$, \\ TRUE)} (Q9)
			(Q8) edge          node[align=center,left, near end] {($\mathit{L.onCreateLoader_{exit}}$, \\ $\mathit{true}$)} (Q9)
			(Q9) edge          node[align=center] {$\epsilon$} (Q10)    
			(Q10) edge         node[align=left, right, very near end] {($\mathit{A.onStart_{exit}}$, $\mathit{true}$)} (Q5)
			
			(Q5) edge[edgeasync, bend left]         node[align=center,swap] {(\footnotesize $\mathit{CList.onClick_{entry}}$, \\ \footnotesize $\mathit{evt = click_{b1}}$)} (Q11)
			(Q11) edge[bend left]         node[align=center] {($\mathit{CList.onClick_{exit}}$, \\ $\mathit{true}$)} (Q5)
			(Q5) edge[edgeasync]     node[align=right, left] {($\mathit{A.onStop_{entry}}$, \\ $\mathit{evt = back\_button}$)} (Q12)
			(Q12) edge[bend left]     node[align=center] {($\mathit{A.onStop_{exit}}$, \\ $\mathit{true}$)} (Q1)
			%            (Q4) edge         node[align=center] {\scriptsize ($L.onCreateLoader_{entry}(cs)$, \\ \scriptsize $cs == initLoader$)} (Q5)
			%            (Q5) edge         node[align=center] {\scriptsize ($L.onCreateLoader_{exit}(cs)$, \\ TRUE)} (Q8)
			%            (Q8) edge         node[align=center,left] {($A.onStart_{exit}$, \\ TRUE)} (Q9)
			%            (Q9) edge[bend left]         node[align=center] {($A\$1.onClick_{entry}$(evt), \\ evt == click(b1))} (Q10)
			%            (Q10) edge[bend left]         node[align=center] {($A\$1.onClick_{exit}$(evt), \\ TRUE)} (Q9)
			%            (Q9) edge     node[align=center] {($A.onStop_{entry}$, \\ TRUE)} (Q11)
			%            (Q11) edge     node[align=center] {($A.onStop_{exit}$, \\ TRUE)} (Q1)
			;
			\end{tikzpicture}
		}
		\caption{A CCFA for simple app}\label{fig:ccfa}
	\end{subfigure}
	\caption{An example app and its CCFA}~\label{fig:ex}
\end{figure}

\subsection{Studies for Designing Coverage Criteria Based on Callbacks}\label{sec:studies}
To further understand what types of callback are important to test, we performed a set of studies. 
For all the studies, we categorize the callbacks based on the context in which they are connected in the CCFA. The context is defined by the type of transition. For example, in Figure \ref{fig:ccfa}, the callbacks \inlinecode{A.onCreate()} and \inlinecode{A.onStart()} are executed under the context of the event \textit{launch}. Similarly, the callback \inlinecode{L.onCreateLoader()} is executed under the context of the API call \inlinecode{lm.initLoader()}. We define 3 types of callbacks based on the different kind of contexts found in the CCFA: \textit{EVENT} for callbacks invoked in external events such as GUI, GPS or power button, \textit{CALL} for callbacks invoked synchronously in API methods, and \textit{MSG} for callbacks invoked asynchronously in API methods (\eg the callback \inlinecode{onStartCommand} is executed asynchronously after calling \inlinecode{startService}). 

%We define the context based on the last guard seenThe source of execution for each callback can be an external event (\eg a GUI event, a GPS location update or a tab to the power button) or an API call. All callbacks invoked in external events are invoked asynchronously whereas an API method can execute a callback synchronously or asynchronously (\eg the callback \inlinecode{onStartCommand} is executed asynchronously after calling \inlinecode{startService}). Thus, we have three categories of callbacks: \textit{ASYNC} (asynchronous callbacks executed from external events), \textit{API\_SYNC} (synchronous callbacks executed in API methods) and \textit{API\_ASYNC} (asynchronous callbacks executed in API methods). In the studies, we want to verify whether a type of callback has important behavior that need to be tested. 

We designed our studies based on three intuitions. First, we believe that if there exists {\it valueflow} between two callbacks, we need to test the paths that traverse the inter-callback valueflow, as any mistakes and bugs related to the global valueflow may only be exposed through exercising inter-callback paths. For example, an object may be associated with a source and a sink that are located in different callbacks. To detect the bug where a source is missing or a sink is missing, we need to test the paths that traverse the callbacks. Second, we want to investigate whether there are callbacks frequently invoked together. If so, we need to test such callback sequences to ensure that the frequently occurred behaviors are tested. Third, we need to learn whether there exist bugs whose root causes are related to specific callback sequences. We need to especially test such interactions of callbacks to avoid similar bugs in different apps. In the following, we present our three studies based on the three intuitions respectively.


\paragraph{Study 1: callbacks involved in global valueflow.} 

In this study, we aim to answer:

{\bf RQ1:} does valueflow frequently occur between callbacks?

{\bf RQ2:} what types of callback are involved in inter-callback valueflow?

We performed source sink analysis for the Android apps on 55 apps randomly selected from the Google Play Market\footnote{\url{https://play.google.com}}. We then performed an analysis using the ICFG of the callbacks to determine the callback where the source statement is executed and the callback where the sink statement is executed. An inter-callback source-sink pair occurs when the source is executed in a different callback than the sink. 

{\bf RQ1:} Our results showed that all 55 apps have inter-callback valueflow. From all the source-sink pairs found, 22.76\% are inter-callback. Therefore,  value flows between different callbacks is frequent in apps.

{\bf RQ2:} We found most the value flows between callbacks occur between callbacks of type EVENT. Value flows where the source and sink callbacks where of type EVENT account for 55\% of all the value flows found in the study. We found that most of the callbacks implemented in apps are EVENT callbacks, which means that most of the functionality is related to GUI or the use of external components such as GPS or camera. The second most common case was value flows between CALL callbacks, which account for 34\% of all value flows. We observed that some API methods invoke more than one callback and the share of data between those callbacks is very common in apps. Value flows from callbacks EVENT $\to$ CALL and from callbacks ASYNC $\to$ MSG account for 4\% each one. The rest of the possible combinations account just for 1\% or less.

\paragraph{Study 2: frequent callback sequences in traces.} In this study, we aim to answer:


{\bf RQ1:} what callback sequences frequently occur in traces?
%{\bf RQ1:} does certain callbacks frequently occur together in traces?

%{\bf RQ2:} if so, what types of callbacks are they? are they app-specific?


To identify what sequences of callbacks are most common in apps, we instrumented 5 apps (\textit{ContactsList}, \textit{StandupTimer}, \textit{BARIA}, \textit{JustCraigslist} and \textit{OpenSudoku}) and collected traces by testing the apps manually. We then mine the most common sequences with two callbacks considering the type of callback. 

{\bf RQ1:} We found that from that 64\% of the callbacks sequences include just EVENT callbacks. The rest of the interactions found in the traces account for 21\% between CALL callbacks. Similarly to the first study, most of the sequences mined are related to callbacks invoked in external events. 

\paragraph{Study 3: pairs of callbacks that lead to bugs.}

In this study, we aim to answer:


{\bf RQ1:} how often are the {\it inter-callback bugs} (bugs whose root causes are related to more than one callback) reported?

%{\bf RQ2:}  what types of callbacks are relevant to the inter-callback bugs?
{\bf RQ2:}  what type of callbacks are relevant to the inter-callback bugs?

We performed a bug study on 6 open source apps. We focus on bugs in which the root cause is related the interaction of callbacks. More precisely, when a sequence of callback executions lead the app to crash. For example, a callback sets a variable to null and the next callback tries to use the variable which raises a runtime null pointer exception. Our methodology was to focus on crashes in the apps. We filter all the closed bugs by using the following keywords: crash, NPE, exception and runtime exception. Then, we manually inspected the bugs to determine the root cause. If the root cause involve interaction of callbacks, then we identify the set of callback interactions needed to trigger the bug. 

Table \ref{tab:bugstudy} shows the results of the study. The classification is based on the type of callbacks involve in the bug. The column \textit{Analyzed} shows the number of bugs we manually studied after filtering by keywords. The column \textit{Matched} shows the number of bugs that match our criteria for inter-callback bugs. The column \textit{EVENT} contain the number of bugs which involve at least one callback of type EVENT. We apply the same metric for columns \textit{CALL} and \textit{MSG}. Most of the bugs reported under EVENT include both EVENT and MSG callbacks (they are also reported under MSG). We found just 2 bugs in which the callbacks involved were just of type EVENT. For bugs involving callbacks of type CALL, we found 2 bugs which also involve EVENT callbacks and 2 bugs which just involve CALL callbacks. 


%Note that if the bug requires callback interactions \textit{(Asynchronous, Follows)} and \textit{(Synchronous,Follows)} we categorize it as the behavior to trigger the bug can be cover by C1. If the bug includes an \textit{(Synchronous, Invocation)} interaction, then we categorize it as C2. Lastly, if the bug includes an \textit{(Asynchronous, Invocation)}, the behavior can only be covered by C3. 

\begin{table}[!ht]
	\centering
	\caption{Bug Study Results}\label{tab:bugstudy}
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{|l|r|r|r|r|r|} \hline
			App & Analyzed & Matched & EVENT & CALL & MSG \\ \hline \hline
			ConnectBot & 9 & 5 & 2 & 0 & 4 \\ \hline
			FileDownloader & 12 & 2 & 1 & 1 & 1 \\ \hline
			AntennaPod & 133 & 5 & 4 & 0 & 5 \\ \hline
			cgeo & 273 & 4 & 2 & 0 & 4 \\ \hline
			Wordpress & 315 & 5 & 1 & 2 & 2 \\ \hline
			Ankidroid & 784 & 5 & 2 & 1 & 4 \\ \hline
			\textbf{Total} & \textbf{1526} & \textbf{26} & \textbf{12} &  \textbf{4} & \textbf{20} \\ \hline
		\end{tabular}
	}
\end{table}

{\bf RQ1:} Inter-callback bugs were frequent among all apps. We found a total of 26 bugs related to inter-callbacks apps in 1526 bugs studied. 

{\bf RQ2:} Our results shows that most of the bugs found include callbacks invoked asynchronously in API methods. Most of these bugs are race conditions between other callbacks of type MSG or callbacks of type EVENT. We also found that for some cases, callbacks invoke synchronously can also be prompt to faults.  

%The most relevant interactions were EVENT callbacks. We see that the main cause of these bugs is the lack of knowledge of all possible callback paths that can be executed when there are other asynchronous callbacks. 

\paragraph{Conclusions of the Studies} In studies 1 and 2 we found that the most of the data is shared between callbacks and the callback interactions involve callbacks invoked in external events or windows (EVENT type). This tells us that the majority of the app implementation is related to GUI (including windows and GUI event handlers) and external events related to components of the phone such as GPS, camera, etc. However, our bug study shows that the callbacks invoke in API methods are prompt to introduce faults. Callbacks invoke asynchronously in API methods are prompt to introduce concurrency faults. Sequences of methods (specially pair of methods) have been used before for coverage criteria designed to detect concurrency bugs \cite{choudharyconcurrency, tasharoficoncurrency}. Thus, we consider that callback sequences are an adequate metric to cover concurrency faults in Android apps. 

We design different coverage criteria founded in our studies. Since most of the data shared between callbacks and the most common interactions among apps include just callbacks of type EVENT, we design a coverage criterion that include callbacks of type EVENT. Because some of the faults found include both EVENT and CALL or EVENT and MSG types of callbacks, we design coverage criterion to model these interactions also. 

\subsection{Designing Testing Criteria Based on Callbacks}
We have identified 3 types of callbacks based on the control change between two callbacks. We have used examples to show these interactions are feasible. In this section, we develop three testing criteria, namely {\it C1}, {\it C2} and {\it C3}, that aim to cover these interactions. Shown in Table \ref{tab:coveragecriteria}, the criteria is designed in a way that {\it C1} is the weakest, {\it C2} is stronger by including one more type of callbacks, and {\it C3} is the strongest that aim for covering all types of callbacks.
% In the following, we further show that there are different sets of app behaviors that can be covered by C1, C2 and C3. 

%The main hypothesis of this paper is that current GUI event-based and structural coverage criteria are not the best metrics to verify the adequacy of a test suite. We want to test the hypothesis that a more specialized coverage criteria is needed besides GUI event-based ones. We design 3 coverage criteria, one more complex than the other to observe whether the behaviors added are important to identify faults. Each coverage criterion is defined based on the type of callbacks interactions they cover. Table \ref{tab:coveragecriteria} shows the 3 different coverage criteria we define and the callbacks interaction that each of them cover. 

%Each coverage criterion is defined based on type of interactions they cover. 

%Therefore, by covering just certain changes of control between callbacks, a coverage criterion focus on specific behaviors in the app. Table \ref{tab:coveragecriteria} shows 4 coverage criteria we define. 

\begin{table}
	\centering
	\caption{Testing Criteria based on Callback Interactions}\label{tab:coveragecriteria}
	%	\resizebox{\columnwidth}{!}{
	\begin{tabular}{|l|l|} \hline
		Name & Callback Types  \\ \hline  \hline
		C1 & EVENT \\ \hline
		C2 & EVENT, CALL \\ \hline
		C3 & EVENT, CALL, MSG  \\ \hline
	\end{tabular}
	%	}
\end{table}


\textbf{C1. } Coverage criterion C1 is designed to cover sequences of callbacks of type EVENT, meaning all callbacks related to windows and external events. As we observed in the studies shown in Section \ref{sec:studies}, most of data shared between callbacks involve just EVENT callbacks and the most common sequences of callbacks found in traces were also from EVENT callbacks. A test suite that satisfies C1 must cover the majority of the apps since as we observed, apps are mostly composed by EVENT callbacks. 

The behaviors covered by C1 are close to the behaviors of a GUI model. The difference with a coverage criterion based on GUI callbacks is that C1 also requires to exercise the behaviors between callbacks invoked in other kind of external events besides GUI events. For example, in Figure \ref{fig:example3} we present an app which registers listeners callbacks for two buttons (lines~7 and 8) and a callback to receive GPS location updates (line~9). Figure \ref{fig:ccfaexample3} shows the CCFA that is built for the app. Assuming we are going to test sequences of two callbacks, test suites have to test the following sequences of callbacks for \inlinecode{A.onCreate()}: 
\begin{itemize}
	\item $\mathit{A.onCreate_{entry}} \to \mathit{A.onCreate_{exit}} \to \mathit{Button1.onClick_{entry}}$
	\item $\mathit{A.onCreate_{entry}} \to \mathit{A.onCreate_{exit}} \to \mathit{Button2.onClick_{entry}}$
	\item $\mathit{A.onCreate_{entry}} \to \mathit{A.onCreate_{exit}} \to$ \\ $\mathit{LocList.onLocationUpdate_{entry}}$
\end{itemize}

Similarly, the sequences for callbacks \inlinecode{Button1.onClick}, \inlinecode{Button2.onClick} and \inlinecode{LocList.onLocationUpdate} include the all the permutations between these 3 callbacks.  We observe that to satisfy C1 for this app, location events have to happen before or after a GUI callback. An event-based coverage criterion just have to cover the combination of the two GUI callbacks. Therefore, C1 can have more behaviors to test. 

\begin{figure}
	\centering
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\resizebox{0.85\columnwidth}{!}{
			%\lstset{basicstyle=\listingsfont, numbers=left, language=Java}
			\lstinputlisting{code/example3.java}
		}
		\caption{Source code of a simple Android app including GPS events\label{fig:example3}}		
	\end{subfigure}
	\begin{subfigure}[b]{\columnwidth}
		\centering
		\resizebox{0.85\columnwidth}{!}{
			\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2.3cm,
			semithick]
			%\tikzstyle{every state}=[fill=cadmiumgreen,draw=none,text=white]
			
			\node[initial,state, accepting] (Q1)                    {$q_1$};
			\node[state]         (Q2)  [below of=Q1] {$q_2$};
			\node[state]         (Q3)  [below of=Q2] {$q_3$};
			\node[state]         (Q4)  [left of=Q3, xshift=-0.9cm] {$q_4$};
			\node[state]         (Q5)  [right of=Q3, xshift=0.9cm] {$q_5$};
			\node[state]         (Q6)  [below of=Q3,yshift=-0.9cm] {$q_6$};
			
			\path
			(Q1) edge         node[align=center] {(\footnotesize $\mathit{A.onCeate_{entry}}$, $\mathit{evt = launch}$)} (Q2)
			(Q2) edge		  node[near start] {(\footnotesize $\mathit{A.onCreate_{exit}}$, $\mathit{true}$)} (Q3)
			%			
			(Q3) edge[bend right,swap]		  node[align=center] {(\footnotesize $\mathit{Button1.onClick_{entry}}$, \\ \footnotesize $\mathit{evt = click_{b1}}$)} (Q4)
			(Q4) edge[bend right, swap]		  node[align=center] {(\footnotesize $\mathit{Button1.onClick_{exit}}$, \\ \footnotesize true)} (Q3)
			
			(Q3) edge[bend left]		  node[align=center] {(\footnotesize $\mathit{Button2.onClick_{entry}}$, \\ \footnotesize $\mathit{evt = click_{b2}}$)} (Q5)
			(Q5) edge[bend left]		  node[align=center] {(\footnotesize $\mathit{Button2.onClick_{exit}}$, \\ \footnotesize $\mathit{true}$)} (Q3)
			
			(Q3) edge[bend right, swap]		  node[align=center,near end] {(\footnotesize $\mathit{LocList.onLocationUpdate_{entry}}$, \\ \footnotesize $\mathit{evt = location}$)} (Q6)
			(Q6) edge[bend right, swap]		  node[align=center,near start] {(\footnotesize $\mathit{LocList.onLocationUpdate_{exit}}$, \\ \footnotesize $\mathit{true}$)} (Q3)
			;
			\end{tikzpicture}
		}
		\caption{A CCFA for the app}\label{fig:ccfaexample3}
	\end{subfigure}
	\caption{An app with Location Callbacks}\label{fig:applocation}
\end{figure}

\textbf{C2.} Coverage criterion C2 adds the set of callbacks invoked synchronously in API methods (API\_SYNC) on top of C1. In the studies in Section \ref{sec:studies}, we found that a third of the data shared between callbacks were found in API\_SYNC callbacks. Additionally, we found important bugs related to these callbacks. To generate sequences involving API\_SYNC callbacks, we can use the CCFA. For example, from the callback \inlinecode{A.onStart} shown in the CCFA in Figure \ref{fig:ccfa}, there are 3 sequences of callbacks of length 2 that can be generated: 
\begin{itemize}
	\item $\mathit{A.onStart_{entry}} \to \mathit{L.onCreateLoader_{entry}}$
	\item $\mathit{A.onStart_{entry}} \to \mathit{A.Start_{exit}} \to \mathit{A.onStop_{entry}}$
	\item $\mathit{A.onStart_{entry}} \to \mathit{A.Start_{exit}} \to \mathit{CList.onClick_{entry}}$
\end{itemize}

Since the callback \inlinecode{A.onStart()} calls the API method \textit{LoaderManager.initLoader()} and this method invokes synchronously \inlinecode{L.onCreateLoader()}, there is a sequence between the two entry points of these callbacks. Nonetheless, there is a path in the app in which \inlinecode{A.onStart()} does not call \textit{LoaderManager.initLoader()}. That is why, there are sequences of callbacks from \inlinecode{A.onStart()} to \inlinecode{CList.onClick()} and \inlinecode{A.onStop()}. A test suite need to cover all the paths that call API methods that invoke callbacks. 

Even when a test suite reaches an API call that invokes callbacks synchronously, there are some cases in which the API method can execute different callbacks under different states of the system. As we presented in the example showed in Figures \ref{fig:filedownloder610code} and \ref{fig:filedownloader610subseq}, for some API methods, the app needs certain state to trigger all the possible callbacks invoked in a method (in this case, an older app already installed in the system). The sequences to test from the callback \inlinecode{FDService.onCreate()} are the following: 
\begin{itemize}
	\item $\mathit{FDService.onCreate_{entry}} \to \mathit{DBHelper.onCreate_{entry}}$
	\item $\mathit{FDService.onCreate_{entry}} \to \mathit{DBHelper.onUpgrade_{entry}}$
	\item $\mathit{FDService.onCreate_{entry}} \to \mathit{DBHelper.onOpen_{entry}}$
\end{itemize}

To completely test these sequences, the app has to be freshly installed and also has to update an older version of the app previously installed in the phone. Thus, to satisfy C2, apps have to be tested under special environments. 

\textbf{C3.} Coverage criterion C3 adds sequences that involve callbacks invoked asynchronously in API methods (API\_ASYNC). Some of API methods that make asynchronous calls include  \inlinecode{Handler.sendMessage} and \inlinecode{Context.startService}. Most of the bugs we found in Section \ref{sec:studies} that involve API\_ASYNC callbacks were race conditions.  Concurrency bugs related to asynchronous callbacks invoked in API calls have been studied before \cite{raceandroidmaiya, raceandroidhsiao, racebielik}. They can be frequent in apps that include several asynchronous callbacks. For example, the bug presented in Figures \ref{fig:chanu140code} and \ref{fig:chanu140subseq} involve EVENT callbacks and API\_ASYNC callbacks. The possible sequences of callbacks from \inlinecode{CaptureList.onClick()} are the following:
\begin{itemize}
	\item $\mathit{CaptureList.onClick_{entry}} \to \mathit{CaptureList.onClick_{exit}} \to$ \\ $\mathit{CaptureList.onClick_{entry}}$
	\item $\mathit{CaptureList.onClick_{entry}} \to  \mathit{CaptureList.onClick_{exit}} \to$ \\ $\mathit{CamAct\$3.onPictureTaken_{entry}}$
\end{itemize}

%For example, in the issue \#3991 for the app \textit{cgeo}~\cite{cgeo3991}, there is data race condition between a tab to the back button and an asynchronous callback executed using the API method \inlinecode{Handler.sendMessage}. Thus, the asynchronous interactions between external events and also between callbacks invoke in API calls are important to cover.

Test suites that satisfy C3 must exercise the concurrent behavior that an app can present from not just external events, but the interaction of external events and callbacks invoked asynchronously in API methods. We explain how to generate sequences involving these callbacks in Section \ref{sec:computing}. 
%C2 adds the set of callback interactions \textit{(Synchronous, Invocation)} on top of C1. The advantage of considering \textit{(Synchronous, Invocation)} interactions if a test suite misses the execution of an API call that invokes callbacks synchronously, it will be reflected in all the callback interactions the API method executes. However, an event-based coverage criteria, would not have knowledge about these execution paths. Even when a test suite reaches an API call that invokes callbacks synchronously, there are some cases in which the API method can execute different callbacks under different states of the system. As we presented in the example showed in Figures \ref{fig:filedownloder610code} and \ref{fig:filedownloader610subseq}, for some API methods, the app needs certain state to trigger all the possible callbacks invoked in a method (in this case, an older app already installed in the system). Another example can be seen in the API method \inlinecode{LoaderManager.initLoader()}. This method will the execute callback \inlinecode{LoaderCallbacks.onCreateLoader()} if the data the loader has not been created or \inlinecode{LoaderCallbacks.onLoad()} if the loader has been created and data was already loaded. Thus, the different callbacks interactions in an API method, provide knowledge about the different paths that need to be cover in the framework.
%As shown in Section \ref{sec:motivation}, API methods can execute different sequences of callbacks when executed under different environments. The bug can be missed if testing does not sufficiently cover different paths of the relevant part of the framework, triggered by different environments. 
